A Neural Benders Decomposition for the Hub Location Routing Problem

In this study, we propose an imitation learning framework designed to enhance the Benders decomposition method. Our primary focus is addressing degeneracy in subproblems with multiple dual optima, among which Magnanti-Wong technique identifies the non-dominant solution. We develop two policies. In the first policy, we replicate the Magnanti-Wong method and learn from each iteration. In the second policy, our objective is to determine a trajectory that expedites the attainment of the final subproblem dual solution. We train and assess these two policies through extensive computational experiments on a network design problem with flow subproblem, confirming that the presence of such learned policies significantly enhances the efficiency of the decomposition process.

==> ALNS.tex <==
In certain problems, a local search that makes iteratively small changes to a feasible solution within a neighborhood structure, often fails to find other promising parts of the solution's space. The so-called Large Neighborhood Search (LNS) as introduced in \cite{Shaw1997ANL}, was proposed to answer this issue. LNS is grounded on the idea of partially destroying a currently feasible solution and repairing it through some local search; if any improvement is observed, we decide whether to accept it or not. The idea behind such a destruction phase is that by introducing more than just a small change in every iteration, we may end up finding better and promising feasible solutions by sampling from across the solution space. When the number of these destruction and repair operators increases and the operators compete with each other in their potential to contribute in finding better solutions, we refer to this as a Variable Neighborhood Search-like algorithm (VNS-Like) (see for instance \cite{Ropkealns2005TRSC}). In this VNS-like algorithm, the choice of operators to be applied in every iteration is adaptively determined by the weights/awards attributed to their performance and it is guided by the statistics that is gathered during the search process.\\

\cite{mladenovic1997variable} follows similar agenda. In Variable Neighborhood Search (VNS), we alternate between different \emph{improvement} methods which are mainly based on exploring different neighborhoods in a systematic way, trying to find better solutions, as well as a \emph{shaking} method in charge of injecting noises (perturbation/diversification) in the solution process, avoiding the situation of prematurely meeting any of the stopping conditions.\\

Regarding the so-called \emph{Improvement} methods, during the solution procedure, several systematic ways of exploring neighborhoods are proposed in the literature which some of them are mentioned below: \emph{Composite (Nested) VND} (see e.g., \cite{rphub}, where full Nested VND was applied for the first time); \emph{sequential Variable Neighborhood Descent (seqVND)} (see e.g., \cite{VNSAnn} for more details); and \emph{Mixed Nested VND} (see e.g., \cite{ilic2010general} as an application of Mixed Nested VND) from among others.  The \emph{well-known} General Variable Neighborhood Search (GVNS) \citep{VNSAnn} is one of the major references that incorporates advanced procedures in the improvement phase.

%The \emph{Shaking} procedure, which may correspond to the destruction operator(s) of the ALNS, is applied to help escape from local optima where improvement procedures  get stuck and the search process stagnates. %Traditionally, two parameters are being used as stopping criteria: $maxIter$, the \emph{maximum number of iterations} and  $t_{max}$, the \emph{maximum allowed CPU time}. \\
Interested readers to this subject are referred to \citep{VNSAnn,mladenovic2016less} for an overview of successful applications of VNS variants for solving various optimization problems.


%Our approach that is elaborated in the following integrates an MIP solver as a part of the solution process whether for solving the purely continuous part of the problem or for recreating a partially ruined solution resulted by the operators.  In such case, we use CPLEX as a component of the solution method. In this way, one may wish to consider this approach a matheuristic-like method.\\



%\textcolor{red}{for all VNd and GVNS etc we should give some references}


\subsection{Initial solution}\label{Initial-DSTS}
In every feasible solution to the DSTS, there are two classes of trailers. The ones that will be served and those that cannot be scheduled because no compatible time slot was found to serve trucks during the planning horizon. Therefore, we divide the them in three categories: 1) served trucks 2) unserved ones, and 3) those being excluded from the solution.\\

Three simple/naive ways to generate an initial solutions follow:

\begin{itemize}[-]\label{heurs}
\item  \textsc{ArrivalVertical}: From the list of trailers, one trailer per time is added to every dock door in a circular way as long as the time window and the planning horizon is respected on every machine.

\item \textsc{ArrivalHorizontal}: One dock door at a time is being planned. The first inbound trailer is allocated to the first dock door and at the same dock door, the next task to be added is a trailer whose arrival time is the closest to the end time of the previous one. This is to be repeated until we fill the planning horizon for the current dock door and before we start planing for the next dock door.
\item \textsc{MinArrivalVertical}: From the list of trailers \emph{sorted by their arrival times}, one trailer is added to every dock door in a circular way as long as the time window and the planning horizon is respected.
\end{itemize}


\subsubsection{Destruction operators}\label{sec:destruction}
Two destruction operators can be envisaged.

\paragraph{\textsc{InterDockRandomRemoval}} $\alpha$ percent of the whole trailers scheduled on different dock doors are dropped from the current feasible solution. These trailers are removed from the set of served ones and added to the list of excluded trailers.\

\paragraph{\textsc{DoublyRandomRemoval}} In contrast to the previous operator, the trailers to be removed are a subset with the cardinality equal to $\beta$ percent of the trailers belonging to a randomly selected dock doors. The trailers are removed from the set of served trailers and are added to the list of excluded ones.\

\paragraph{\textsc{IntraDockRandomRemoval}} For a given dock door, $\gamma$ percent of trailers belonging to it will be dropped from the dock door. The trailers are removed from the set of served trailers and are added to the list of excluded ones.\


\paragraph{\textsc{WipeDock}} All trailers completed on a given dock door are removed from the dock door and are added to the list of excluded trailers.\\


It must be noted that in all these cases, the resulting solution does remain a feasible solution.\


\subsubsection{Repair operators}\label{sec:repair}
Two repair operators are proposed here.

\paragraph{\textsc{InsertFromUnserveds}} From a list of \emph{unserved} inbound trailers sorted by their arrival time, we try to insert, in a greedy manner, new trailers from the top of the list between/before/after the tailers being served in the current solution.\


\paragraph{\textsc{InsertFromUnservedsWithLookAhead}} From a list of \emph{unserved} inbound trailers sorted by their service plus docking times, we try to insert one or two trailers between/before/after the trailers being served in the current solution, in a way to fill the idle gaps.\\


\subsubsection{Local Search Operator}\label{sec:localsearch}


\paragraph{\textsc{ReplaceWithUnserved}} For every trailer in the list of \emph{unserved} ones, we examine the improving potential of it replacing a truck in the current solution.\


\paragraph{\textsc{SwapTrailers}} In every solution, we examine the possibility of swapping trailers between two dock doors.\

\subsubsection{Adaptive weight adjustment}\label{sec:adaptiveweight}
A transition matrix is considered where $T^t=[\tau^t_{{o_i}{o_j}}]$ represents the weight of applying operator $o_i$ after operator $o_j$, at time $t$. This weight is calculated by:
\begin{align}
\tau^{t+1}_{o_i~o_j} = \tau^{t}_{o_i~o_j} - \frac{f^{out} - f^{in}}{f^{in}} \nonumber
\end{align}
wherein $f^{in}$ and $f^{out}$ are the objective values resulted by the application of operators $o_i$ and $o_j$, before and after operator $o$ is applied. \\

Clearly, transition from any operator to a destruction operator results in negative values. However, this is not an issue in this algorithm as we allow both positive and negative weights for every operator. The initial weights are chosen randomly.\

\subsubsection{Acceptance Criteria}\label{sec:acceptance}
\cite{Shaw1997ANL} proposed to only accept improving solutions while \cite{Ropkealns2005TRSC} suggested using simulated annealing with linear cooling scheme. In the case of this problem, our initial computational experiments confirm that the earlier method performs better. Therefore, we only accept improving solutions.




\subsubsection{Stopping criteria}\label{sec:termination}
From among many possible stopping criteria we opt for the one that measures the vanishing differences (increasing similarity) between  matrices $T$ in consecutive iterations. For calculating the differences, one may use any of the following metrics:
\begin{align}
   & d_1(\mathbf{T^{t-1}}, \mathbf{T^{t}}) = \sum_{i=1}^n \sum_{j=1}^n |\tau_{o_i~o_j}^{t-1} - \tau_{o_i~o_j}^{t}| \label{eq:difference}\\
   & d_2(\mathbf{T^{t-1}}, \mathbf{T^{t}}) = \sqrt{\sum_{i=1}^n \sum_{j=1}^n (\tau_{o_i~o_j}^{t-1} - \tau_{o_i~o_j}^{t})^2} \\
   & d_\infty(\mathbf{T^{t-1}}, \mathbf{T^{t}}) = \max_{1 \le i \le n}\max_{1 \le j \le n} |\tau_{o_i~o_j}^{t-1} - \tau_{o_i~o_j}^{t}| \\
   & d_n(\mathbf{T^{t-1}}, \mathbf{T^{t}}) = \max\{ \|(\mathbf{\mathbf{T^{t-1}}} - \mathbf{\mathbf{T^{t}}})\mathbf{x}\| : \mathbf{x} \in \mathbb{R}^n, \|\mathbf{x}\| = 1 \}
\end{align}


Here, we opted for \eqref{eq:difference} for measuring similarity of matrices.\\

The overall process terminates once no improvement is observed for $N^{max_{NonI}^{iter}}$ consecutive iterations and the matrices start to look very similar for a relative differences (i.e. $\frac{d_*}{\mathbf{T^{t}}}$) below an assumed threshold $\epsilon$. \\


%\subsubsection{Feasibility and objective value}
%Feasibility of a move can be checked at different stages. It is identified if an incompatibility is observed at the time windows level. Yet, there are situations where the infeasibility can be identified at the time of calculating the objective function. Our initial computational experiments confirmed that a hashing mechanism contributes extraordinarily in the overall efficiency of the approach.


\subsection{Steps of the proposed VNS-like algorithm}
\autoref{alg:ALNS} represents the major steps of our VNS-like approach. An initial solution constructed in \autoref{Initial-DSTS} will be the input to the VNS-like algorithm. The destruction, repair and local search operators are chosen from among those in \autoref{sec:destruction}, \autoref{sec:repair} and \autoref{sec:localsearch} called in this order. If any improvement is observed the best-found solution is updated. As we always accept an improving solution, the starting solution of the next iterations will be the best-known feasible solution of all the previous iterations. The overall process is over as soon as one of the termination criteria in \autoref{sec:termination} is met.\\


\begin{algorithm}
\caption{VNS-like algorithm} \label{alg:ALNS}
\begin{algorithmic}[1]
\Procedure{VNS}{$s\in Solution$}%\Comment{Sequential Variable  Neighborhood Decent}
\State $s_{best} = s$\;
\Repeat
\State $s_0 = s$;
\State select and apply the best destruction operator on $s_0$\; \label{op1}
\State select and apply the best repair operator on $s_0$\;\label{op2}
\State select and apply the best local search operator on $s_0$\;\label{op3}
\If {$f(s_0) < f(s_{best})$}
    $s_{best} = s_0$\;
\EndIf
\If {$accept(s_0, s)$}
    $s = s0$\;
\EndIf
\State update transition table, $T$\;
\Until{stop-criterion met}\\\;
\Return {$s_{best}$}\;
\EndProcedure\;
\end{algorithmic}
\end{algorithm}





%
%
%
%\State $s \leftarrow$ seqVND(s) \Comment{improvement using the seq. VND elaborated in \autoref{SeqVNS}}\;
%%\State $s$=$T\leftarrow Improvement\_procedure(T)$\;
%\Repeat
%\State $k \leftarrow 1$\;
%\While{$k \leq k_{max}$}
%    \State $s' \leftarrow Shake(s,k)$ \;
%    %\State $T''\leftarrow Improvement\_procedure(T')$\;
%    \State $s'' \leftarrow  seqVND(s')$ \Comment{improvement using the Adaptive VND elaborated in \autoref{SeqVNS}}\;
%    \State $k \leftarrow k+1$\;
%    \If{$v(s'')> v(s)$}
%        \State $s \leftarrow s''$;$k\leftarrow 1$
%    \EndIf
%\EndWhile
%\Until{{\tt CpuTime()}$ > t_{max}$}
%\State $t \leftarrow $ {\tt CpuTime()};
%\State \textbf{return} $s$%\Comment{The gcd is b}






==> DW.tex <==
Let $\mathcal{K}$ be the set of columns. We refer to the element of this set (which are generated by the pricing problem) as \emph{pseudo-schedules} as they do not necessarily represent  complete or even feasible schedules (complete solution).\\

A Dantzig-Wolfe reformulation of the problem follows:

%\begin{align}
%%\small
%min \:      &\sum_{t\in \mathcal{T}}\sum_{i,j \in \mathcal{J}^+} \sum_{k=1}^{\mathcal{K}}\lambda_{k}\left(f_i(t+p_i+\delta_i))\widehat{x}_{ijt}^{k}\right) + \sum_{i\in\mathcal{J}}g_i{z_i}\label{eq:rmp:obj1}\\
%            s.\:t.\:\nonumber\\
%            &   \sum_{r\in \mathcal{R}}\sum_{i\in \mathcal{J}^\circ:j\neq i}\sum_{t=r_{i}}^{|{\mathcal{T}}|}\left(\sum_{k=1}^{\mathcal{K}}\lambda_{k}\widehat{x}_{ijt}^{k}\right)+z_j =1,   &   j\in\mathcal{J},\label{eq:rmp:eq1}\\
%            &   \sum_{r\in \mathcal{R}}\sum_{i\in \mathcal{J}^\circ:j\neq i}\sum_{t=r_{j}}^{|{\mathcal{T}}|}\left(\sum_{k=1}^{\mathcal{K}}\lambda_{k}\widehat{x}_{jit}^{k}\right) +z_i=1,   &                                      i\in\mathcal{J},\label{eq:rmp:eq2}\\
%            &   \sum_{k=1}^{\mathcal{K}}\lambda_{k} =1,   &   \label{eq:rmp:eq3}                                \\
%            & x_{ijkt} - \sum_{k=1}^{\mathcal{K}}\lambda_{k}\widehat{x}_{ijt}^{k} = 0\label{eq:rmp:eq4}\\
%            &   \lambda_{k}\geq 0,  &   \label{eq:rmp:eq5}\\
%            & x \in \{0,1\}^ {|\mathcal{J}^\circ|\times|\mathcal{J}^\circ|\times||\mathcal{T}|}\label{eq:rmp:vars}.
%\end{align}
%We can safely remove the $z_i$ variables from this formulation and re-write the master problem as:

\begin{align}
%\small
min \:      & ~\sum_{d \in \mathcal{D}} ~\sum_{t \in \mathcal{T}} ~\sum_{i, j \in \mathcal{J}^\circ} ~\sum_{k=1}^{\mathcal{K}} \lambda_{k} \left(f_j (t - r_j)) \widehat{x}_{ijdt}^{k} \right) \label{eq:rmp:obj}\\
%            \eqref{eq:rmp:obj1} \label{eq:MP:obj}\\
            s.\: t.\: \nonumber\\
            (u^1_j):~~~~&   ~\sum_{d \in \mathcal{D}}~\sum_{i \in \mathcal{J}^\circ: ~j \neq i} ~\sum_{t = r_{i}}^{|{\mathcal{T}}|} \left( \sum_{k = 1}^{\mathcal{K}} \lambda_{k} \widehat{x}_{ijdt}^{k} \right) \leq 1,   &   j \in \mathcal{J}, \label{eq:rmp:eq3}\\
            (u^2_j):~~~~&   ~\sum_{d \in \mathcal{D}}~\sum_{i \in \mathcal{J}^\circ: ~j \neq i} ~\sum_{t = r_{j}}^{|{\mathcal{T}}|} \left( ~\sum_{k = 1}^{\mathcal{K}} \lambda_{k} \widehat{x}_{jidt}^{k} \right) \leq 1,   &                                      j \in \mathcal{J}, \label{eq:rmp:eq4}\\
            (\alpha):~~~~&   ~\sum_{k = 1}^{\mathcal{K}} \lambda_{k} = 1,   &   \label{eq:rmp:eq5}                                \\
            (v_{ijkt}):~~~~& x_{ijkt} - ~\sum_{k = 1}^{\mathcal{K}} \lambda_{k} \widehat{x}_{ijt}^{k} = 0,   & i \in \mathcal{J^\circ}, j \in \mathcal{J} \label{eq:rmp:eq6}\\
            &   \lambda_{k} \geq 0, t \in \mathcal{T} &   \label{eq:rmp:eq7}\\
            & x \in \{0,1\}^ {|\mathcal{J}^\circ| |\mathcal{J}^\circ| |\mathcal{D}| |\mathcal{T}|} \label{eq:rmp:vars}.
\end{align}

Now, let remove $z_j$ from the model \eqref{eq:arcTimeIndex:obj1} - \eqref{eq:arcTimeIndex:vars} by replacing it with $1 - ~\sum_{d \in \mathcal{D}} ~\sum_{i \in \mathcal{J}^\circ: ~j \neq i} ~\sum_{t \in \mathcal{T}} x_{jidt}$ in our following pricing problem. Moreover, as the dual values associated to the constraints \eqref{eq:arcTimeIndex:eq1} and \eqref{eq:arcTimeIndex:eq2} are unsigned, we turn these two constraints into half-space constraints \eqref{eq:rmp:eq3} and \eqref{eq:rmp:eq4} without any harm. We also introduce $h_i, i\in\mathcal{J}$ taking 1, if trailer $i$ is served, 0 otherwise.\\



Given the dual values associated with the constraints in \eqref{eq:rmp:eq3}-\eqref{eq:rmp:eq6}, namely $u^1_j$, $u^2_j$, $\alpha$ and $v_{ijkt}$, then the Pricing Problem (PP) is as follows:

\begin{align}
%\small
min \:      & ~\sum_{ i \in \mathcal{J^\circ}, j \in \mathcal{J}, d \in \mathcal{D}, t \in \mathcal{T}} ~f_j(t - r_j) x_{ijdt} + ~\sum_{ j \in \mathcal{J}} ~g_j ( 1 - ~\sum_{ d \in \mathcal{D}}~\sum_{ i \in \mathcal{J}^\circ: ~j \neq i}~\sum_{ t \in \mathcal{T}} ~x_{jidt}) \nonumber\\
& - ~\sum_j ~u^1_j ~\left( \sum_{ d \in \mathcal{D}}~\sum_{ i \in \mathcal{J}^\circ: ~j \neq i}~ \sum_{ t \in \mathcal{T}} ~x_{ijdt} ~\right) - ~\sum_j ~u^2_j ~\left( ~\sum_{ d \in \mathcal{D}}~\sum_{ i \in \mathcal{J}^\circ: ~j \neq i} ~\sum_{ t \in \mathcal{T}} ~x_{jidt} \right) \nonumber\\
&~ - \sum_{ i \in \mathcal{J}^\circ, j \in \mathcal{J}, d \in \mathcal{D}, t \in \mathcal{T}} ~v_{ijdt} x_{ijdt} - \alpha
\label{eq:PP:obj1}\\
%min \:      & \sum_{j \in \mathcal{J}^+}\left( \sum_{r\in \mathcal{D}}\sum_{i\in \mathcal{J}} \sum_{t}tx_{ijdt}-r_i\right)
%\label{eq:arcTimeIndex:obj2}\\
            s.\:t.\:\nonumber\\
      &   ~\sum_{ j \in \mathcal{J}}~\sum_{t\in \mathcal{T}} ~x_{0jdt} \leq |\mathcal{D}|,     &  \forall ~d \in \mathcal{D} \label{eq:PP:eq1}\\
      %
            &   ~\sum_{ i \in \mathcal{J}}~\sum_{ t \in \mathcal{T}} x_{i0dt} \leq  |\mathcal{D}|,     &     \forall ~d \in \mathcal{D}, \label{eq:PP:eq2}\\
       %
            &   ~\sum_{ i \in \mathcal{J}^\circ}~\sum_{ t \in \mathcal{T}} (x_{ijdt} - x_{jidt} ) = 0,           &   \forall ~d \in \mathcal{D}, \forall ~j \in \mathcal{J}   \label{eq:PP:eq3}\\
       %
            &   ~-\sum_{ d \in \mathcal{D}}~\sum_{ i \in \mathcal{J}}~\sum_{ j \in \mathcal{J}: ~j \neq i} ~x_{ijdt} + ~\sum_{ i \in \mathcal{J}} ~h_i = |\mathcal{D}|,           &     \label{eq:PP:eq4}\\
       %
            &   ~\sum_{ d \in \mathcal{D}} ~x_{ijdt} \leq h_j,           &     \forall ~i \in \mathcal{J}^\circ, j \in \mathcal{J}, \forall ~t \in \mathcal{T} \label{eq:PP:eq5}\\
%       %
            &   ~\sum_{ j \in \mathcal{J}^\circ}~\sum_{ t \in \mathcal{T}} ~x_{ijdt} \geq  h_i,           &     \forall ~i \in \mathcal{J}\label{eq:PP:eq6}\\
       %
            &\eqref{eq:arcTimeIndex:eq61}, \eqref{eq:rmp:vars}, \eqref{eq:arcTimeIndex:symmetry}\nonumber,\nonumber\\
            & h_j  \in \{0,1\}^ {|\mathcal{J}|}
\end{align}
%where
%
Constraints \eqref{eq:PP:eq1} (\eqref{eq:PP:eq2}) ensure that no more than $\mathcal{D}$ arcs could leave from (arrive to)  the dummy node (trailer). Constraints \eqref{eq:PP:eq3} guarantee the flow conservation at every intermediate node (trailer). Constraints \eqref{eq:PP:eq4} ensure that in any pseudo-schedule, the number of trailers being served minus the number of arcs connecting real trailers among themselves is equal to the number of dock doors. Constraints \eqref{eq:PP:eq5} indicate that no arc enters a trailer node, unless the trailer is among the ones to be served. Constraints \eqref{eq:PP:eq6} make sure that at some point in time an arc would enter into node $j$ if trailer $j$ is among the trailers to be served.\\

%We refer to a solution to \eqref{eq:PP:obj1}-\eqref{eq:PP:eq5}, \eqref{eq:arcTimeIndex:eq61}, \eqref{eq:rmp:vars} and \eqref{eq:arcTimeIndex:symmetry} for every dock door as a \emph{pseudo-schedule} as it does not necessarily represent a complete (or even a feasible) schedule.
%\\
%Moreover, $h_i^t$ refers to the number of dock doors, active serving a trailer at any moment $t$.
%
%However, due to the fact that the pricing problem objective coefficients can be negative, often we do end up with situation where the constraint \eqref{eq:MP:eq3} and \eqref{eq:MP:eq4} are highly violated. In such situations, to avoid several non-improving iterations, we add constraint that try to control this violation from being very extreme.
%
%
%Given that the number of compatible tasks to every workover rig $r\in\mathcal{R}$ is limited to a set $|\mathcal{J}^r|$ (knowing that $0\in \mathcal{J}^r$, i.e. 0 is compatible to every workover rig), we can write the following constraints:
%
%\begin{align}
%&\sum_{i,j \in \mathcal{J}^\circ}\sum_{t=0}^T x_{ij}^t \leq |\mathcal{J}^r|
%\end{align}
%%|T|- |M| - 1
\subsection{Branch and cut for the pricing subproblem}
%One of the main questions that may appear here is whether we could split the pricing problem per every dock? or if we could have one convexity constraints of form \eqref{eq:MP:eq6} per dock? It should be noted that as the cost structure does not depend on the docks and is the same across all the docks, it has been observed through computational experiments that such subproblems will often all produce identical solutions, in particular in the very early iterations. It will take quite a few iterations until the dual values of the restricted master problem constraints would be distributed in a way to give different problems. That is why we opted to not split the subproblem per docks. One may also notice that the final cost of a solution needs to take into account penalties for the unserved trucks and therefore, this cost structure is not a additive function wherein $f(x+y) = f(x)+f(y)$. While there are workarounds to address these issues, our computational experiments did not confirm the viability of those approaches.\\\
%
%Ir order to solve the pricing problem we have kept constraints \eqref{eq:arcTimeIndex:eq1}, \eqref{eq:arcTimeIndex:eq2} in the pricing problem, which present some properties similar to the assignment problem constraints. We then separated constraints \eqref{eq:arcTimeIndex:eq61}  and symmetry elimination constraints \eqref{eq:arcTimeIndex:symmetry} as well \eqref{eq:valid:1} and \eqref{eq:valid:3} at every integer node where one or more of these cuts were violated.

%The valid inequalities from among those in as well as those in \autoref{sec:valid} can be separated. Given that we have original space variables in both restricted master problem and the pricing problem, separating valid inequalities of the original space becomes rather easy and the modifications imposed on the subproblem as a consequence of adding cuts to the master problem will only modify the objective function in the pricing problem.


\paragraph{Cutting plane}

Some valid inequalities have been identified, which are separated at every integer solution along the Branch-and-Bound tree of the pricing problem. On this way, at every node of the Branch-and-Bound tree, by calling the \emph{cutcallback} procedure, the algorithm verifies whether there exists any violated constraint or. Found violated constraints will be inserted to the model as new cuts to help removing the current fractional solution from the feasible region. \\
Constraints below are involved in this cutting plane algorithm:

\begin{align}
&   ~\sum_{t \in \mathcal{T}} ~(x_{ijdt} + x_{i0dt} + x_{j0dt}) \leq 2, &   \forall ~i,j \in \mathcal{J}, \forall ~j \neq i, d \in \mathcal{D}\\
&   ~\sum_{t \in \mathcal{T}} ~(x_{ijdt} + x_{0idt} + x_{0jdt}) \leq 2, &   \forall ~i,j \in \mathcal{J}, \forall ~j\neq i, d \in \mathcal{D}
\end{align}
%The number of arcs
\begin{align}
&   ~\sum_{t \in \mathcal{T}} ~\sum_{m \in \mathcal{J}: ~m \neq i, m \neq j} ~(x_{midt} + x_{jmdt}) \geq h_i  + h_j , &   \forall ~i,j \in \mathcal{J}, \forall ~j \neq i, d \in \mathcal{D}
\end{align}


\paragraph{Branching strategy} Our extensive computational experiments suggested emphasizing on rapid improvement of lower bound (breadth-first search).

\subsection{Branch, price and cut}
The proposed D-W decomposition provides the building blocks of our branch, price and cut (more precisely branch-and-price as no cutting is done at the master problem level).
\paragraph{Branching}
Branching is done on the original variables $x_{ijkt}$ as per constraints \eqref{eq:rmp:eq7}:

\begin{align}
  & x_{ijdt} - \sum_{k=1}^{\mathcal{K}}\lambda_{k}\widehat{x}_{ijdt}^{k} = 0, &   \forall i,j,d,t. \label{eq:rmp:eq7}\\
  & x \in \{0,1\}^ {|\mathcal{J}^\circ||\mathcal{J}^\circ||\mathcal{D}||\mathcal{T}|}\nonumber.
\end{align}

\paragraph{Warm-start with an initial column}
It is rather straightforward to create the first feasible solution to the DSTS problem. One naive way, which delivers relatively good solution is the following: we sort the trailers by their arrival time and by starting from the top of the sorted list, iterating over dock doors and allocate one trailer per time to every dock door in a circular way as long as the feasibility is respected.









==> Largest.tex <==
Inst.Name	& Obj.Val.	& \#Nodes		&Status	&CPUTime(sec.)	&\#n.Cols	&\#PrIter		&Served/Total \%  &CPUTime(Heu.)\\
\specialrule{.2em}{.1em}{.1em}
\endfirsthead
\specialrule{.2em}{.1em}{.1em}
Inst.Name	& Obj.Val.	& \#Nodes		&Status	&CPUTime(sec.)	&\#n.Cols	&\#Pr.Iter		&Served/Total \%  &CPUTime(Heu.)\\
\specialrule{.2em}{.1em}{.1em}
\endhead
tf\_20\_tr\_60&	970.00&	1&	Opt.&	45.89&	6&	2&	98.33	&	6.70	\\
tf\_20\_tr\_65&	3312.00&	1&	Opt.&	0.97&	2&	2&	90.77	&	0.36	\\
tf\_20\_tr\_70&	1678.00&	1&	Opt.&	20.38&	12&	2&	95.71	&	6.96	\\
tf\_20\_tr\_75&	3835.00&	1&	Opt.&	22.21&	9&	2&	90.67	&	7.26	\\
tf\_20\_tr\_80&	4998.00&	1&	Opt.&	19.97&	13&	2&	88.75	&	7.47	\\
tf\_20\_tr\_85&	8325.00&	1&	Opt.&	69.87&	12&	2&	83.53	&	3.17	\\
tf\_20\_tr\_90&	11966.00&	1&	Opt.&	32.83&	11&	2&	77.78	&	4.66	\\
tf\_20\_tr\_95&	14343.00&	1&	Opt.&	67.67&	22&	2&	74.74	&	6.80	\\
tf\_20\_tr\_100&	14843.00&	1&	Opt.&	32.07&	12&	2&	75	&	2.55	\\
\hline										
tf\_22\_tr\_66&	2810.00&	1&	Opt.&	1.16&	2&	2&	92.42	&	0.12	\\
tf\_22\_tr\_71&	636.00&	1&	Opt.&	6.75&	3&	2&	98.59	&	1.52	\\
tf\_22\_tr\_76&	4651.00&	1&	Opt.&	14.17&	6&	2&	89.47	&	2.73	\\
tf\_22\_tr\_81&	4328.00&	1&	Opt.&	10.15&	6&	2&	90.12	&	7.49	\\
tf\_22\_tr\_86&	6761.00&	1&	Opt.&	106.85&	28&	2&	87.21	&	5.25	\\
tf\_22\_tr\_91&	11550.00&	1&	Opt.&	6.39&	7&	2&	79.12	&	6.12	\\
tf\_22\_tr\_96&	11529.00&	1&	Opt.&	34.41&	15&	2&	78.12	&	1.65	\\
tf\_22\_tr\_101&	14719.00&	1&	Opt.&	48.08&	13&	2&	77.23	&	3.40	\\
tf\_22\_tr\_106&	14597.00&	1&	Opt.&	83.75&	21&	2&	75.47	&	1.54	\\
\hline										
tf\_24\_tr\_72&	2103.00&	1&	Opt.&	10.33&	11&	2&	94.44	&	2.21	\\
tf\_24\_tr\_77&	2995.00&	1&	Opt.&	13.29&	25&	2&	94.81	&	7.40	\\
tf\_24\_tr\_82&	2487.00&	1&	Opt.&	31.07&	15&	2&	96.34	&	1.39	\\
tf\_24\_tr\_87&	2241.00&	1&	Opt.&	16.04&	9&	2&	95.4	&	7.19	\\
tf\_24\_tr\_92&	5563.00&	1&	Opt.&	59.91&	22&	2&	89.13	&	1.13	\\
tf\_24\_tr\_97&	6618.00&	1&	Opt.&	14.21&	13&	2&	88.66	&	5.90	\\
tf\_24\_tr\_102&	10951.00&	1&	Opt.&	15.32&	16&	2&	81.37	&	6.07	\\
tf\_24\_tr\_107&	11778.00&	1&	Opt.&	70.68&	13&	2&	81.31	&	1.66	\\
tf\_24\_tr\_112&	17201.00&	1&	Opt.&	122.13&	25&	2&	75	&	4.04	\\
tf\_24\_tr\_117&	17498.00&	1&	Opt.&	209.52&	18&	2&	75.21	&	3.48	\\
\hline										
tf\_26\_tr\_78&	2918.00&	1&	Opt.&	1.04&	2&	2&	94.87	&	0.71	\\
tf\_26\_tr\_83&	1098.00&	1&	Opt.&	27.26&	16&	2&	98.8	&	7.24	\\
tf\_26\_tr\_88&	2306.00&	1&	Opt.&	3.53&	6&	2&	95.45	&	1.62	\\
tf\_26\_tr\_93&	4770.00&	1&	Opt.&	3.36&	4&	2&	91.4	&	3.07	\\
tf\_26\_tr\_98&	2793.00&	1&	Opt.&	40.24&	13&	2&	94.9	&	4.37	\\
tf\_26\_tr\_103&	6530.00&	1&	Opt.&	159.15&	11&	2&	88.35	&	5.69	\\
tf\_26\_tr\_108&	11418.00&	1&	Opt.&	36.86&	23&	2&	80.56	&	4.61	\\
tf\_26\_tr\_113&	11586.00&	1&	Opt.&	58.58&	15&	2&	82.3	&	7.65	\\
tf\_26\_tr\_118&	12496.00&	1&	Opt.&	215.97&	18&	2&	80.51	&	2.66	\\
tf\_26\_tr\_123&	16306.00&	1&	Opt.&	284.05&	12&	2&	76.42	&	1.52	\\
tf\_26\_tr\_128&	20994.00&	1&	Opt.&	337.83&	22&	2&	72.66	&	3.96	\\
\hline										
tf\_28\_tr\_84&	851.00&	1&	Opt.&	2.15&	3&	2&	98.81	&	0.89	\\
tf\_28\_tr\_89&	3340.00&	1&	Opt.&	4.73&	8&	2&	93.26	&	2.94	\\
tf\_28\_tr\_94&	1570.00&	1&	Opt.&	4.93&	6&	2&	97.87	&	0.18	\\
tf\_28\_tr\_99&	3971.00&	1&	Opt.&	97.86&	25&	2&	93.94	&	6.04	\\
tf\_28\_tr\_104&	5776.00&	1&	Opt.&	378.73&	21&	2&	90.38	&	2.25	\\
tf\_28\_tr\_109&	7318.00&	1&	Opt.&	71.08&	11&	2&	88.99	&	1.32	\\
tf\_28\_tr\_114&	6770.00&	1&	Opt.&	167.84&	17&	2&	90.35	&	2.42	\\
tf\_28\_tr\_119&	13697.00&	1&	Opt.&	62.50&	20&	2&	80.67	&	5.23	\\
tf\_28\_tr\_124&	15245.00&	1&	Opt.&	139.10&	20&	2&	78.23	&	7.53	\\
tf\_28\_tr\_129&	16532.00&	1&	Opt.&	151.20&	19&	2&	79.07	&	15.45	\\
tf\_28\_tr\_134&	17441.00&	1&	Opt.&	583.40&	16&	2&	78.36	&	60.99	\\
tf\_28\_tr\_139&	21982.00&	1&	Opt.&	186.44&	22&	2&	73.38	&	41.06	\\
\hline										
tf\_30\_tr\_90&	2110.00&	1&	Opt.&	1.76&	2&	2&	96.67	&	0.63	\\
tf\_30\_tr\_95&	2200.00&	1&	Opt.&	16.40&	10&	2&	96.84	&	2.57	\\
tf\_30\_tr\_100&	3039.00&	1&	Opt.&	1049.11&	19&	2&	96	&	6.35	\\
tf\_30\_tr\_105&	4528.00&	1&	Opt.&	97.05&	14&	2&	93.33	&	19.95	\\
tf\_30\_tr\_110&	5797.00&	1&	Opt.&	16.86&	9&	2&	90.91	&	17.82	\\
tf\_30\_tr\_115&	7430.00&	1&	Opt.&	33.73&	13&	2&	89.57	&	7.29	\\
tf\_30\_tr\_120&	8141.00&	1&	Opt.&	46.12&	12&	2&	87.5	&	4.25	\\
tf\_30\_tr\_125&	9358.00&	1&	Opt.&	240.27&	43&	2&	86.4	&	7.31	\\
tf\_30\_tr\_130&	13734.00&	1&	Opt.&	1009.80&	13&	2&	83.85	&	2.36	\\
tf\_30\_tr\_135&	19677.00&	1&	Opt.&	64.90&	15&	2&	74.81	&	5.38	\\
tf\_30\_tr\_140&	17305.00&	1&	Opt.&	3286.31&	19&	2&	77.86	&	5.56	\\
tf\_30\_tr\_145&	20641.00&	1&	Opt.&	1847.73&	31&	2&	76.55	&	6.50	\\
tf\_30\_tr\_150&	23810.00&	1&	Opt.&	325.07&	23&	2&	72.67	&	6.01	\\
\hline										
tf\_32\_tr\_96&	1546.00&	1&	Opt.&	2.80&	2&	2&	97.92	&	1.76	\\
tf\_32\_tr\_101&	1533.00&	1&	Opt.&	13.34&	9&	2&	98.02	&	7.07	\\
tf\_32\_tr\_106&	1611.00&	1&	Opt.&	4.79&	6&	2&	98.11	&	2.92	\\
tf\_32\_tr\_111&	3411.00&	1&	Opt.&	9269.34&	26&	2&	95.5	&	66.96	\\
tf\_32\_tr\_116&	6838.00&	1&	Opt.&	42.37&	10&	2&	90.52	&	4.68	\\
tf\_32\_tr\_121&	7396.00&	1&	Opt.&	135.38&	21&	2&	89.26	&	3.96	\\
tf\_32\_tr\_126&	10214.00&	1&	Opt.&	7720.07&	17&	2&	86.51	&	7.02	\\
tf\_32\_tr\_131&	9544.00&	1&	Opt.&	379.84&	21&	2&	87.79	&	7.90	\\
tf\_32\_tr\_136&	13746.00&	1&	Opt.&	3240.46&	26&	2&	83.09	&	1.19	\\
tf\_32\_tr\_141&	14857.00&	1&	Opt.&	13962.96&	17&	2&	82.27	&	6.98	\\
tf\_32\_tr\_146&	18929.00&	1&	Opt.&	246.22&	27&	2&	77.4	&	5.81	\\
tf\_32\_tr\_151&	22127.00&	1&	Opt.&	1635.46&	14&	2&	74.83	&	6.03	\\
tf\_32\_tr\_156&	22582.00&	1&	Opt.&	248.55&	19&	2&	74.36	&	3.40	\\
\hline										
tf\_34\_tr\_102&	3577.00&	1&	Opt.&	1.95&	2&	2&	94.12	&	0.47	\\
tf\_34\_tr\_107&	2802.00&	1&	Opt.&	55.43&	5&	2&	96.26	&	2.48	\\
tf\_34\_tr\_112&	1269.00&	1&	Opt.&	77.95&	27&	2&	99.11	&	2.08	\\
tf\_34\_tr\_117&	3707.00&	1&	Opt.&	2819.07&	15&	2&	94.87	&	15.67	\\
tf\_34\_tr\_122&	6437.00&	1&	Opt.&	28.45&	13&	2&	91.8	&	17.25	\\
tf\_34\_tr\_127&	6486.00&	1&	Opt.&	107.16&	16&	2&	91.34	&	3.05	\\
tf\_34\_tr\_132&	9623.00&	1&	Opt.&	4391.02&	22&	2&	87.12	&	2.04	\\
tf\_34\_tr\_137&	12657.00&	1&	Opt.&	94.47&	18&	2&	84.67	&	6.80	\\
tf\_34\_tr\_142&	13685.00&	1&	Opt.&	136.32&	12&	2&	84.51	&	7.14	\\
tf\_34\_tr\_147&	13846.00&	1&	Opt.&	10418.44&	29&	2&	83.67	&	7.46	\\
tf\_34\_tr\_152&	18734.00&	1&	Opt.&	1957.39&	18&	2&	78.95	&	7.27	\\
tf\_34\_tr\_157&	18959.00&	1&	Opt.&	842.66&	26&	2&	79.62	&	7.53	\\
tf\_34\_tr\_162&	20619.00&	1&	Opt.&	477.86&	24&	2&	77.78	&	3.77	\\
tf\_34\_tr\_167&	27181.00&	1&	Opt.&	2469.96&	25&	2&	72.46	&	4.56	\\
\hline										
tf\_36\_tr\_108&	1737.00&	1&	Opt.&	14.52&	9&	2&	97.22	&	6.08	\\
tf\_36\_tr\_113&	3083.00&	1&	Opt.&	39.79&	17&	2&	96.46	&	6.70	\\
tf\_36\_tr\_118&	3130.00&	1&	Opt.&	13.16&	8&	2&	95.76	&	6.80	\\
tf\_36\_tr\_123&	2375.00&	1&	Opt.&	45.82&	21&	2&	97.56	&	5.84	\\
tf\_36\_tr\_128&	5768.00&	1&	Opt.&	4114.34&	16&	2&	92.97	&	7.16	\\
tf\_36\_tr\_133&	6968.00&	1&	Opt.&	342.87&	13&	2&	91.73	&	4.30	\\
tf\_36\_tr\_138&	7924.00&	1&	Opt.&	255.87&	14&	2&	90.58	&	7.72	\\
tf\_36\_tr\_143&	10745.00&	1&	{\scriptsize AbrtUsr							
 (0.00)}&	14446.08&	18&	2&	86.71	&	71.04	\\			
tf\_36\_tr\_148&	12854.00&	1&	{\scriptsize AbrtUsr							
 (206.49)}&	14819.20&	31&	2&	84.46	&	22.74	\\			
tf\_36\_tr\_153&	20404.00&	1&	Opt.&	3005.55&	14&	2&	78.43	&	7.39	\\
tf\_36\_tr\_158&	22504.00&	1&	Opt.&	263.03&	22&	2&	74.68	&	5.23	\\
tf\_36\_tr\_163&	18934.00&	1&	Opt.&	655.60&	32&	2&	80.98	&	6.06	\\
tf\_36\_tr\_168&	25932.00&	1&	{\scriptsize AbrtUsr							
 (302.71)}&	16421.30&	30&	2&	74.4	&	55.38	\\			
tf\_36\_tr\_173&	27555.00&	1&	Opt.&	563.60&	20&	2&	72.25	&	14.47	\\
tf\_36\_tr\_178&	29488.00&	1&	{\scriptsize AbrtUsr							
 (0.00)}&	12552.96&	19&	2&	71.35	&	6.22	\\			
\hline										
tf\_38\_tr\_114&	2316.00&	1&	Opt.&	2.82&	2&	2&	96.49	&	1.25	\\
tf\_38\_tr\_119&	921.00&	1&	Opt.&	30.29&	11&	2&	99.16	&	2.90	\\
tf\_38\_tr\_124&	2202.00&	1&	Opt.&	19.93&	17&	2&	97.58	&	7.52	\\
tf\_38\_tr\_129&	6761.00&	1&	Opt.&	57.82&	11&	2&	91.47	&	5.68	\\
tf\_38\_tr\_134&	4178.00&	1&	{\scriptsize FailFeas							
 (356.55)}&	15963.79&	27&	2&	94.78	&	7.37	\\			
tf\_38\_tr\_139&	5270.00&	1&	{\scriptsize AbrtUsr							
 (797.02)}&	14476.57&	24&	2&	94.24	&	6.56	\\			
tf\_38\_tr\_144&	6750.00&	1&	{\scriptsize AbrtUsr							
 (47.69)}&	14501.72&	34&	2&	91.67	&	6.24	\\			
tf\_38\_tr\_149&	8617.00&	1&	Opt.&	281.92&	16&	2&	89.93	&	5.75	\\
tf\_38\_tr\_154&	16153.00&	1&	Opt.&	1641.64&	19&	2&	82.47	&	31.46	\\
tf\_38\_tr\_159&	16050.00&	1&	{\scriptsize AbrtUsr							
 (0.00)}&	7422.39&	35&	2&	82.39	&	5.08	\\			
tf\_38\_tr\_164&	16952.00&	1&	Opt.&	484.44&	18&	2&	82.93	&	3.28	\\
tf\_38\_tr\_169&	20657.00&	1&	Opt.&	676.18&	21&	2&	79.29	&	11.29	\\
tf\_38\_tr\_174&	21276.00&	1&	Opt.&	6059.44&	19&	2&	78.74	&	3.45	\\
tf\_38\_tr\_179&	21823.00&	1&	Opt.&	6238.04&	24&	2&	78.77	&	6.82	\\
tf\_38\_tr\_184&	29133.00&	1&	{\scriptsize AbrtUsr							
 (447.32)}&	14611.69&	32&	2&	72.83	&	5.38	\\			
tf\_38\_tr\_189&	29020.00&	1&	{\scriptsize AbrtUsr							
 (286.73)}&	14485.56&	44&	2&	73.54	&	1.69	\\			
\hline										
tf\_40\_tr\_120&	1791.00&	1&	Opt.&	52.16&	20&	2&	98.33	&	5.70	\\
tf\_40\_tr\_125&	1955.00&	1&	Opt.&	6.04&	4&	2&	97.6	&	2.85	\\
tf\_40\_tr\_130&	3918.00&	1&	Opt.&	4.67&	3&	2&	95.38	&	1.37	\\
tf\_40\_tr\_135&	1542.00&	1&	Opt.&	68.45&	15&	2&	98.52	&	6.89	\\
tf\_40\_tr\_140&	3861.00&	1&	Opt.&	20.63&	8&	2&	95	&	6.28	\\
tf\_40\_tr\_145&	6699.00&	1&	{\scriptsize AbrtUsr							
 (156.67)}&	14840.12&	23&	2&	92.41	&	17.45	\\			
tf\_40\_tr\_150&	8366.00&	1&	Opt.&	1336.33&	32&	2&	91.33	&	12.99	\\
tf\_40\_tr\_155&	12525.00&	1&	Opt.&	531.89&	15&	2&	86.45	&	7.27	\\
tf\_40\_tr\_160&	13896.00&	1&	Opt.&	802.48&	35&	2&	85.62	&	6.55	\\
tf\_40\_tr\_165&	13007.00&	1&	{\scriptsize AbrtUsr							
 (152.10)}&	14506.03&	44&	2&	86.06	&	6.55	\\			
tf\_40\_tr\_170&	18787.00&	1&	{\scriptsize AbrtUsr							
 (535.72)}&	14752.17&	31&	2&	81.18	&	5.73	\\			
tf\_40\_tr\_175&	20877.00&	1&	{\scriptsize AbrtUsr							
 (96.91)}&	14606.47&	37&	2&	79.43	&	5.02	\\			
tf\_40\_tr\_180&	23633.00&	1&	Opt.&	5064.76&	23&	2&	77.22	&	6.10	\\
tf\_40\_tr\_185&	23818.00&	1&	Opt.&	2506.01&	42&	2&	78.38	&	2.13	\\
tf\_40\_tr\_190&	23999.00&	1&	Opt.&	4681.24&	18&	2&	76.84	&	4.52	\\
tf\_40\_tr\_195&	30108.00&	1&	{\scriptsize AbrtUsr							
 (107.24)}&	14496.11&	28&	2&	73.33	&	4.36	\\			
\hline										
tf\_42\_tr\_126&	1982.00&	1&	Opt.&	15.94&	9&	2&	97.62	&	2.90	\\
tf\_42\_tr\_131&	620.00&	1&	Opt.&	71.31&	12&	2&	99.24	&	2.59	\\
tf\_42\_tr\_136&	2119.00&	1&	Opt.&	196.26&	21&	2&	98.53	&	3.75	\\
tf\_42\_tr\_141&	3066.00&	1&	{\scriptsize AbrtUsr (405.96)}&	14934.59&	13&	2&	96.45	&	7.93	\\			
tf\_42\_tr\_146&	4363.00&	1&	Opt.&	734.28&	24&	2&	95.89	&	2.87	\\
tf\_42\_tr\_151&	8697.00&	1&	Opt.&	1412.47&	16&	2&	90.07	&	6.75	\\
tf\_42\_tr\_156&	9646.00&	1&	Opt.&	373.34&	11&	2&	89.1	&	4.15	\\
tf\_42\_tr\_161&	10279.00&	1&	{\scriptsize AbrtUsr (50.11)}&	14793.01&	30&	2&	88.82	&	3.30	\\			
tf\_42\_tr\_166&	12290.00&	1&	Opt.&	4926.42&	48&	2&	87.35	&	6.22	\\
tf\_42\_tr\_171&	15207.00&	1&	Opt.&	530.01&	19&	2&	84.21	&	5.52	\\
tf\_42\_tr\_176&	13685.00&	1&	Opt.&	5958.26&	15&	2&	86.36	&	6.06	\\
tf\_42\_tr\_181&	20275.00&	1&	{\scriptsize AbrtUsr (0.00)}&	7714.94&	11&	2&	80.66	&	2.21	\\			
tf\_42\_tr\_186&	19506.00&	1&	Opt.&	4456.86&	27&	2&	82.26	&	4.54	\\
tf\_42\_tr\_191&	26947.00&	1&	{\scriptsize AbrtUsr (1231.70)}&	14729.70&	14&	2&	76.44	&	6.77	\\			
tf\_42\_tr\_196&	28850.00&	1&	Opt.&	4116.89&	22&	2&	76.02	&	33.98	\\
\hline										
tf\_44\_tr\_132&	125.00&	1&	Opt.&	8.90&	6&	2&	100	&	7.10	\\
tf\_44\_tr\_137&	3826.00&	1&	Opt.&	93.67&	12&	2&	96.35	&	6.53	\\
tf\_44\_tr\_142&	3890.00&	1&	Opt.&	7.54&	5&	2&	95.77	&	4.45	\\
tf\_44\_tr\_147&	3661.00&	1&	Opt.&	149.13&	15&	2&	95.92	&	1.36	\\
tf\_44\_tr\_152&	7621.00&	1&	Opt.&	2455.69&	21&	2&	92.11	&	7.22	\\
tf\_44\_tr\_157&	8029.00&	1&	Opt.&	3325.88&	15&	2&	90.45	&	3.85	\\
tf\_44\_tr\_162&	9602.00&	1&	{\scriptsize AbrtUsr (0.00)}&	6826.91&	39&	2&	91.36	&	7.74	\\			
tf\_44\_tr\_167&	10304.00&	1&	Opt.&	4883.78&	42&	2&	89.22	&	2.61	\\
tf\_44\_tr\_172&	9955.00&	1&	{\scriptsize AbrtUsr (161.36)}&	14646.70&	38&	2&	90.12	&	15.44	\\			
tf\_44\_tr\_177&	12561.00&	1&	{\scriptsize AbrtUsr (0.00)}&	9412.04&	72&	2&	87.57	&	32.17	\\			
tf\_44\_tr\_182&	19685.00&	1&	{\scriptsize AbrtUsr (275.00)}&	18158.12&	45&	2&	82.42	&	11.41	\\			
tf\_44\_tr\_187&	18742.00&	1&	{\scriptsize AbrtUsr (443.78)}&	14922.88&	43&	2&	82.89	&	6.13	\\			
tf\_44\_tr\_192&	21050.00&	1&	Opt.&	3442.52&	28&	2&	80.73	&	6.92	\\
tf\_44\_tr\_197&	21928.00&	1&	{\scriptsize AbrtUsr (15.33)}&	14714.76&	48&	2&	81.73	&	7.08	\\			
\hline										
tf\_46\_tr\_138&	3265.00&	1&	Opt.&	4.15&	2&	2&	95.65	&	1.74	\\
tf\_46\_tr\_143&	4542.00&	1&	Opt.&	5.77&	2&	2&	95.8	&	1.44	\\
tf\_46\_tr\_148&	2762.00&	1&	Opt.&	8.57&	5&	2&	97.97	&	5.23	\\
tf\_46\_tr\_153&	5242.00&	1&	Opt.&	25.70&	6&	2&	94.77	&	7.84	\\
tf\_46\_tr\_158&	1730.00&	1&	{\scriptsize AbrtUsr							
 (432.35)}&	14508.09&	75&	2&	98.73	&	5.45	\\			
tf\_46\_tr\_163&	5792.00&	1&	{\scriptsize AbrtUsr							
 (223.07)}&	14716.14&	53&	2&	94.48	&	4.28	\\			
tf\_46\_tr\_168&	6917.00&	1&	Opt.&	1789.96&	15&	2&	94.05	&	6.66	\\
tf\_46\_tr\_173&	7414.00&	1&	Opt.&	269.35&	21&	2&	92.49	&	4.82	\\
tf\_46\_tr\_178&	11085.00&	1&	{\scriptsize AbrtUsr							
 (1223.16)}&	14656.66&	43&	2&	89.33	&	4.56	\\			
tf\_46\_tr\_183&	13970.00&	1&	{\scriptsize AbrtUsr							
 (458.42)}&	14595.03&	29&	2&	87.43	&	6.91	\\			
tf\_46\_tr\_188&	15983.00&	1&	Opt.&	5284.12&	61&	2&	84.57	&	7.41	\\
tf\_46\_tr\_193&	21324.00&	1&	{\scriptsize AbrtUsr							
 (13.33)}&	14485.80&	46&	2&	81.87	&	7.15	\\			
tf\_46\_tr\_198&	21396.00&	1&	Opt.&	4484.45&	38&	2&	81.82	&	17.23	\\
\hline										
tf\_48\_tr\_144&	2231.00&	1&	Opt.&	4.93&	2&	2&	97.92	&	1.07	\\
tf\_48\_tr\_149&	2459.00&	1&	Opt.&	5.59&	2&	2&	97.32	&	4.35	\\
tf\_48\_tr\_154&	2636.00&	1&	Opt.&	91.33&	21&	2&	98.05	&	1.57	\\
tf\_48\_tr\_159&	2552.00&	1&	Opt.&	190.63&	16&	2&	98.11	&	4.91	\\
tf\_48\_tr\_164&	5393.00&	1&	Opt.&	244.51&	15&	2&	94.51	&	7.68	\\
tf\_48\_tr\_169&	2288.00&	1&	{\scriptsize AbrtUsr							
 (852.72)}&	14473.34&	43&	2&	98.22	&	5.20	\\			
tf\_48\_tr\_174&	6916.00&	1&	{\scriptsize AbrtUsr							
 (62.53)}&	14753.88&	25&	2&	93.68	&	3.75	\\			
tf\_48\_tr\_179&	6839.00&	1&	{\scriptsize AbrtUsr							
 (54.00)}&	14535.07&	23&	2&	93.85	&	2.93	\\			
tf\_48\_tr\_184&	9387.00&	1&	Opt.&	2241.05&	30&	2&	91.3	&	3.11	\\
tf\_48\_tr\_189&	12798.00&	1&	Opt.&	1474.89&	14&	2&	88.89	&	2.87	\\
tf\_48\_tr\_194&	17464.00&	1&	Opt.&	5419.80&	42&	2&	84.02	&	6.21	\\
tf\_48\_tr\_199&	19078.00&	1&	Opt.&	4097.30&	24&	2&	84.42	&	6.98	\\
\hline										
tf\_50\_tr\_150&	1005.00&	1&	Opt.&	20.63&	8&	2&	99.33	&	7.13	\\
tf\_50\_tr\_155&	755.00&	1&	Opt.&	14.69&	8&	2&	99.35	&	1.15	\\
tf\_50\_tr\_160&	3559.00&	1&	Opt.&	18.97&	9&	2&	96.88	&	5.25	\\
tf\_50\_tr\_165&	4666.00&	1&	Opt.&	111.58&	16&	2&	96.36	&	4.20	\\
tf\_50\_tr\_170&	1591.00&	1&	{\scriptsize AbrtUsr							
 (0.00)}&	6170.61&	16&	2&	98.82	&	3.82	\\			
tf\_50\_tr\_175&	6684.00&	1&	{\scriptsize AbrtUsr							
 (129.17)}&	14474.39&	25&	2&	94.29	&	3.80	\\			
tf\_50\_tr\_180&	9352.00&	1&	Opt.&	526.93&	28&	2&	91.67	&	4.04	\\
tf\_50\_tr\_185&	7430.00&	1&	Opt.&	5894.40&	44&	2&	92.97	&	1.21	\\
tf\_50\_tr\_190&	7424.00&	1&	Opt.&	7072.43&	26&	2&	93.16	&	5.95	\\
tf\_50\_tr\_195&	12136.00&	1&	Opt.&	1863.00&	22&	2&	89.23	&	1.04	\\
\hline										
tf\_52\_tr\_156&	2120.00&	1&	Opt.&	8.46&	2&	2&	98.08	&	1.88	\\
tf\_52\_tr\_161&	2945.00&	1&	Opt.&	13.80&	6&	3&	97.52	&	5.28	\\
tf\_52\_tr\_166&	3351.00&	1&	Opt.&	147.85&	19&	3&	97.59	&	6.51	\\
tf\_52\_tr\_171&	2984.00&	1&	Opt.&	998.37&	23&	2&	98.25	&	2.85	\\
tf\_52\_tr\_176&	4510.00&	1&	{\scriptsize AbrtUsr							
 (512.54)}&	10996.61&	31&	2&	95.45	&	2.11	\\			
tf\_52\_tr\_181&	5272.00&	1&	{\scriptsize AbrtUsr							
 (13.70)}&	8640.81&	14&	2&	95.58	&	5.00	\\			
tf\_52\_tr\_186&	7045.00&	1&	{\scriptsize AbrtUsr							
 (382.60)}&	11063.49&	63&	2&	94.09	&	3.66	\\			
tf\_52\_tr\_191&	11506.00&	1&	{\scriptsize AbrtUsr							
 (205.40)}&	11191.65&	47&	2&	91.1	&	4.41	\\			
tf\_52\_tr\_196&	11948.00&	1&	{\scriptsize AbrtUsr							
 (1416.72)}&	11049.73&	18&	2&	90.31	&	2.51	\\			
\hline										
tf\_54\_tr\_162&	1611.00&	1&	Opt.&	5.75&	2&	2&	98.77	&	4.54	\\
tf\_54\_tr\_167&	2594.00&	1&	Opt.&	194.34&	7&	2&	97.6	&	2.61	\\
tf\_54\_tr\_172&	3483.00&	1&	Opt.&	82.39&	12&	3&	97.09	&	6.86	\\
tf\_54\_tr\_177&	4774.00&	1&	Opt.&	8.63&	2&	2&	96.05	&	4.73	\\
tf\_54\_tr\_182&	3531.00&	1&	{\scriptsize AbrtUsr							
 (910.77)}&	10874.43&	44&	2&	97.25	&	4.01	\\			
tf\_54\_tr\_187&	2221.00&	1&	Opt.&	5446.15&	41&	3&	98.4	&	4.36	\\
tf\_54\_tr\_192&	5752.00&	1&	{\scriptsize AbrtUsr							
 (560.51)}&	10911.02&	68&	2&	95.31	&	4.19	\\			
tf\_54\_tr\_197&	8910.00&	1&	{\scriptsize AbrtUsr							
 (873.86)}&	10927.33&	56&	2&	91.88	&	7.00	\\			
\hline										
tf\_56\_tr\_168&	2957.00&	1&	Opt.&	7.76&	2&	2&	97.62	&	5.11	\\
tf\_56\_tr\_173&	1615.00&	1&	Opt.&	44.28&	10&	2&	98.84	&	2.54	\\
tf\_56\_tr\_178&	9417.00&	1&	Opt.&	9.58&	2&	2&	90.45	&	5.81	\\
tf\_56\_tr\_183&	4979.00&	1&	Opt.&	22.30&	6&	3&	96.17	&	6.09	\\
tf\_56\_tr\_188&	5339.00&	1&	Opt.&	5345.24&	29&	2&	95.74	&	4.45	\\
tf\_56\_tr\_193&	3942.00&	1&	Opt.&	3063.59&	27&	2&	97.41	&	3.22	\\
tf\_56\_tr\_198&	3087.00&	1&	{\scriptsize AbrtUsr							
 (804.27)}&	11171.79&	63&	2&	97.47	&	4.11	\\			
\hline										
tf\_58\_tr\_174&	4036.00&	1&	Opt.&	11.57&	2&	2&	97.13	&	3.09	\\
tf\_58\_tr\_179&	168.00&	1&	Opt.&	9.61&	2&	2&	100	&	1.78	\\
tf\_58\_tr\_184&	3164.00&	1&	Opt.&	145.84&	19&	2&	97.83	&	2.32	\\
tf\_58\_tr\_189&	5142.00&	1&	Opt.&	232.53&	12&	3&	96.3	&	3.11	\\
tf\_58\_tr\_194&	4725.00&	1&	Opt.&	2897.87&	16&	3&	96.91	&	1.77	\\
tf\_58\_tr\_199&	7515.00&	1&	{\scriptsize AbrtUsr							
 (461.79)}&	10858.78&	59&	2&	94.97	&	1.40	\\			
\hline										
tf\_60\_tr\_180&	4088.00&	1&	Opt.&	12.28&	5&	2&	96.67	&	1.98	\\
tf\_60\_tr\_185&	4171.00&	1&	Opt.&	8.81&	2&	2&	96.76	&	4.82	\\
tf\_60\_tr\_190&	2025.00&	1&	Opt.&	19.71&	7&	3&	98.95	&	6.42	\\
tf\_60\_tr\_195&	3738.00&	1&	Opt.&	9.69&	2&	2&	97.44	&	3.93	\\


==> TimeArcIndex.tex <==

                                                             %          %\todo[inline,color=yellow!50,bordercolor=red]{}
%            \todobluedefined[,,caption={When no cost is associated with the installation of hub edges then  \dots}]{When no cost is associated with the installation of hub edges then the resulting hub-level network tends to be complete. }
%            %\todo[inline,color=blue!40]{If all the flow dependent variables move to the subproblem, the master problem does not have any objective function. }
%            %\todo[inline,color=green!30]{Suggestion: we could probably consider a sort of cost for the hub-level edges to not motivate the completeness and at the same time we have an objective function for the problem. Then if we move the flow-based constraints to the subproblem, and master problem takes into account the design variables/constraints, we have an objective function for it and the dual values would be more meaningful.}
\textbf{Dock Scheduling and Truck Sequencing Problem (DSTS)}\
\begin{align}
                                                                                                                 %\small
min \:      & \sum_{i \in \mathcal{J^0}}~\sum_{j \in \mathcal{J}}~\sum_{d \in \mathcal{D}}~\sum_{t\in \mathcal{T}}  ~x_{ijdt} (t-r_j)f_j + \sum_{j\in \mathcal{J}} ~g_jz_j
                                                                                          \label{eq:arcTimeIndex:obj1}\\
%min \:      & \sum_{j \in \mathcal{J}^+}\left( \sum_{r\in \mathcal{D}}\sum_{i\in \mathcal{J}} \sum_{t}tx_{ijdt}-r_i\right)
                                                                                         %\label{eq:arcTimeIndex:obj2}\\
                                                                                                     s.\:t.\:\nonumber\\
&   \sum_{j\in \mathcal{J}}~\sum_{t\in \mathcal{T}} ~x_{0jdt}+x_{00d0} = 1,     &       \forall ~d \in \mathcal{D},\label{eq:arcTimeIndex:eq1}\\
&   \sum_{i\in \mathcal{J}}~\sum_{t\in \mathcal{T}} ~x_{i0dt}+x_{00d0} = 1,           &       \forall d\in\mathcal{D},\label{eq:arcTimeIndex:eq2}\\
&   \sum_{d\in \mathcal{D}}~\sum_{i\in \mathcal{J}^0:j\neq i}~\sum_{t\in \mathcal{T}}~x_{ijdt} + z_j =1,   &   j\in\mathcal{J}, \label{eq:arcTimeIndex:eq3}\\
&   \sum_{d\in \mathcal{D}}~\sum_{i\in \mathcal{J}^0:j\neq i}~\sum_{t\in\mathcal{T}}~x_{jidt} + z_j=1,   &                                      j\in\mathcal{J}, \label{eq:arcTimeIndex:eq4}\\
                            %            &   x_{ijdt}\leq  {\sum_{l\in\mathcal{J} }} x_{jld~t} +x_{j~0~d~t}, \nonumber\\
%            & &   \forall t\in \mathcal{T}, r\in\mathcal{D}, i\in\mathcal{J}^+, j\in\mathcal{J}:j\neq i,t\geq \max\{r_i+p_i+\delta_i,  r_j\}\label{eq:arcTimeIndex:eq5}\\
%%            &   x_{ijrt}\leq \underset{t-t_{ij}-p_i \geq 0} {\sum_{l\in\mathcal{J}^+ }} x_{lir~t-d_{ij}-p_i} ,   &   \forall t\in \mathcal{T}, r\in\mathcal{R}, i\in\mathcal{J}, j\in\mathcal{J}^+:j\neq i,\label{eq:arcTimeIndex:eq6}\\
% %           &   \sum_{r\in\mathcal{R}}\sum_{j\in\mathcal{J}^+:j\neq i} \sum_{t\in\mathcal{T}} x_{ijrt} = 1,          & \forall i\in\mathcal{J},\label{eq:arcTimeIndex:eq6}\\
%%            &   \sum_{i\in\mathcal{J}}\sum_{t\in \mathcal{T}}x_{0irt} = 2,        &   \forall r\in\mathcal{R},\label{eq:arcTimeIndex:eq7}\\
                %%            %&   x_{ijrt} \in \mathbb{B} &   \forall i,j\mathcal{J}, t\in \mathcal{T}, r\in\mathcal{R}
%%%            &   \sum_{j\in \mathcal{J^\circ}}\sum_{t\in \mathcal{T}}x_{ijdt} + \sum_{t\in \mathcal{T}}x_{00dt} \leq 1 , & \forall i\in \mathcal{J}, d\in\mathcal{D},\label{eq:arcTimeIndex:eq5}\\
                                                                                                                      %%
& x_{ijdt} \leq \sum_{l\in \mathcal{J}^\circ:l \neq i , l\neq j} ~\sum_{t'\in \mathcal{T}, t'\geq \max \{r_l, r_{j}+ p_{j}+ \delta_{j}, t+p_j+ \delta_j\}} x_{jldt'}         & \forall ~d\in \mathcal{D}, i\in \mathcal{J}^\circ, j \in \mathcal{J}, t\in \mathcal{T}: j \neq i ,\label{eq:arcTimeIndex:eq61}\\
                                                                                                                      %%
%& x_{ijdt} \geq \sum_{t'\leq \min^\circ\{d_l, d_{i}+p_{i}+\delta_{i},t-p_i-\delta_i, |\mathcal{T}|\}} \sum_{l\in \mathcal{J}^\circ:l\neq i , l\neq j}x_{jldt'}         & \forall d\in \mathcal{D}, j\in \mathcal{J}^\circ, i \in \mathcal{J}, t\in \mathcal{T}: j\neq i ,\label{eq:arcTimeIndex:eq62}\\
                                                                                                                      %%
                                                                                                              % Symmetry
%            & x_{i0dt} \leq \sum_{l} x_{l~i~k~ t - p_i - \delta_i}         & \forall d\in \mathcal{D}, i \in \mathcal{J}, t\in \mathcal{T}: j\neq i ,\label{eq:arcTimeIndex:eq62}\\
                                                                                                                      %%
          %            & x_{ijdt} = 0  & \forall d\in \mathcal{D}, i,j\neq i \in\mathcal{J}, t\in \mathcal{T}\nonumber\\
                           %            &   & (i>0 , ( t> d_j, j\neq 0)\vee (t<r_j) \vee (t<r_i+p_i+\delta_i)\nonumber\\
                                          %            &   & (i=0 , ( t> d_j \vee  t<r_j) ,\label{eq:arcTimeIndex:eq7}\\
                                                                                                                      %%
%            & x_{ijdt} \leq  y_{jt'}    &   \forall  d\in \mathcal{D}, i\in \mathcal{J}^\circ, j \in \mathcal{J}, t\in \mathcal{T}, \nonumber\\
                 %            &   & t'\in\{t+\delta_j+1,\dots, t+\delta_j+p_j \}: j\neq i,\label{eq:arcTimeIndex:eq71}\\
                                                                                                                      %%
%            & \sum_{t\in \mathcal{T}:r_j+\delta_j<t\leq d_j} y_{jt} + p_j z_j \leq p_j,& \forall j \in \mathcal{J},\label{eq:arcTimeIndex:eq72}\\
                                                                                                                      %%
%      &y_{jt}^s  \leq g^s_j, &  \forall t \in \mathcal{T},  \forall j \in \mathcal{J}, s\in \mathcal{S},\label{eq:arcTimeIndex:eq81}\\
                                                                                                                      %%
               %      &\sum_{s\in \mathcal{S}} g^s_j \leq 1, &  \forall j \in \mathcal{J},\label{eq:arcTimeIndex:eq82}\\
                                                                                                                      %%
%      &\sum_{ j \in \mathcal{J}}y_{jt}^s  rp_j^s\leq R^p_j, & \forall t\in \mathcal{T}, s\in \mathcal{S}\label{eq:arcTimeIndex:eq91}\\
%      &\sum_{ j \in \mathcal{J}}y_{jt}^s re_j^s \leq R^e_j, & \forall t\in \mathcal{T}, s\in \mathcal{S}\label{eq:arcTimeIndex:eq92}\\
%     &\sum_{ j \in \mathcal{J}}y_{jt}^s  rv_j^s \leq R^v_j, & \forall t\in \mathcal{T}, s\in \mathcal{S}\label{eq:arcTimeIndex:eq93}\\
                                                                                                                      %%
                                                                                                                      %%
                                                                                                                      %%
&   x \in \{0,1\}^ {|\mathcal{J}^\circ| \times |\mathcal{J}^\circ| \times |\mathcal{D}| \times| \mathcal{T}|}, ~z \in \{0,1\}^ {|\mathcal{J}|}. \label{eq:arcTimeIndex:vars}
\end{align}

The objective function \eqref{eq:arcTimeIndex:obj1} accounts for minimizing the cost of trailers waiting to receive services, as well as the penalty cost of having unfulfilled services.
Constraints \eqref{eq:arcTimeIndex:eq1} ensure that for every dock door, either it starts serving a trailer (let say trailer $j\in\mathcal{J}$); or $x_{00d0}=1$ means that trailer $0$ is started being served after trailer $0$ and its service operation is terminated at time $0$ (the dummy trailer that is served before and after all sequences of served trailers at every dock door).  %If a real truck $i\neq 0$ is received by a dock, then such a first truck on every dock $d$ does not start before $r_i+p_0+d_{i}$ which accounts for the earliest arrival time plus docking and process time of dummy truck $0$.
The last trailer on every dock door is actually the dummy trailer ($0$), which is executed after the last real trailer ($i\in\mathcal{J}$ for $i \neq 0$) on that dock. %Such a truck does not occur during  $[0,r_i+p_0+\delta_0]$, evidently.
This is ensured in constraints \eqref{eq:arcTimeIndex:eq2}. Constraints  \eqref{eq:arcTimeIndex:eq3} ensure that a real trailer (as $j$, if $j \neq 0$) will start at some point in time after another trailer $i\in\mathcal{J}^\circ$ finishes on one of the available dock doors; otherwise it is considered as an unserved trailer. %However, this cannot start earlier than $r_i + p_0+\delta_0$.
Analogously, constraints  \eqref{eq:arcTimeIndex:eq4} ensure that a real trailer $j$ ($j \neq 0$) is followed by another trailer $i$ ($i\in\mathcal{J}^0$) on a dock, otherwise it is considered as a trailer that has not been served. 
% and this cannot occur within $[0,r_i+p_0+\delta_0]$. \\
%For task $j$ executed after a real task $i$ on dock $d$  and time $t$ there must be a consecutive task $l\in\mathcal{J}^\circ$,  which starts no earlier than $t'=\max\{r_l, r_{j}+p_{j}+\delta_{j},t+p_j+\delta_j\}$. This has been ensured by constraints \eqref{eq:arcTimeIndex:eq5}.
%Constraints \eqref{eq:arcTimeIndex:eq5} ensure that no sub-tour will occur in the sequence of trucks being served by a dock. Such a sub-tour would resemble a variable $x_{00d*}$ indicating that the dock is not serving any truck while having a set of tasks associated with the dock $d$ being planned in a cyclic manner.
Constraints \eqref{eq:arcTimeIndex:eq61} ensure that on a given dock door $d$ and at a given period $t$, the trailer following trailer $j$ must be provided enough time for docking activity and processing time, and indeed if its time window allows its service. This set of constraints play the role of sub-tour elimination in this problem. Such a sub-tour would resemble variable $x_{00d*}$ indicating that the dock door is not serving any trailer while having a set of tasks associated with dock door $d$ being planned in a cyclic manner.



%Constraints \eqref{eq:arcTimeIndex:eq71} ensure that truck $j$ receives services following a resource allocation scenario. Constraints \eqref{eq:arcTimeIndex:eq72} guarantee that the resources in a scenario are engaged to serve truck $j$ no more than $p_j$ period of time in a row. Constraints \eqref{eq:arcTimeIndex:eq81}-\eqref{eq:arcTimeIndex:eq82} make sure that only one resource allocation scenario can be used. Constraints \eqref{eq:arcTimeIndex:eq91}- \eqref{eq:arcTimeIndex:eq93} ensure that under any resource allocation scenario, the resource capacity is respected at every period.

%Constraints \eqref{eq:arcTimeIndex:eq7}  fixes to zero, some variables  that can never be one in any feasible solution of the problem instance.\\

%Every machine $j$ is initially located at origin $0$. Constraints \eqref{eq:arcTimeIndex:eq1} indicate that one machine $j\in \mathcal{J}$ is chosen as the first task on machine $r$ and this task %starts as soon as machine $r$ arrives to $j$.\\
%Constraints \eqref{eq:arcTimeIndex:eq2} ensure that one task is executed only one unique machine. For the ease of modeling, $x_{0jr0}=1$ if $j$  is the first task on machine $r$. Constraints %\eqref{eq:arcTimeIndex:eq3} guarantee this. \\
%At every point in time $t$ for the task $i$ on the machine $r$, the number of well executed before task $i$ (at $t-d_{ji}-p_{j}$ for some $j$)  is equal to the number of task executed after it  $i$ (at $t+d_{ij'}+p_{i}$ for some $j'$). This includes the case of $j=j'=0$. Constraints \eqref{eq:arcTimeIndex:eq4} guarantee this. \\
%Every task $j:j\neq 0$ is executed one a unique machine $r$ after another task $j$ (including $0$) in the time interval during $t=\min\{d_{0j:j}\in \mathcal{J}\}$ and $T-d_{ij}-p_j$. Constraints %\eqref{eq:arcTimeIndex:eq5} stands to ensure this.\\
%Constraints \eqref{eq:arcTimeIndex:eq6} ensure that for every non-dummy task $i\in\mathcal{J}$ there is subsequent task on a unique machine at certain time $t$ .\\
%Constraints \eqref{eq:arcTimeIndex:eq7} indicates that on every machine $r$, except for variable $x_{0jr0}=1$ for some task $j$,  there is only one other variable which precisely determines at %which point time $t$ the task $j$ can be started as the first task on machine $r$.





==> literature.tex <==
%Related problems in cross docking in the areas such as: 1) locational analysis and facility layout design, 2) truck dock assignment, 3) vehicle routing, 4) truck scheduling, 6) resource scheduling and, 7) packing/unpacking have received an increasing attention during the last decade.\\
The problem of dock scheduling and truck sequencing arising in cross docks has been an active research area over the last decade. Interested readers are referred to the surveys (\cite{Boysen2010413}, \cite{gu2007research}, \cite{van2012cross}) that are devoted to the assignment, scheduling and the resource management problem in cross docks.


%However, taking into account different levels of details (particularly regarding time) in modeling has led to models, which range from those similar to variants of classical assignment problem to those resembling  the variants of scheduling problems. \
%\subsection{truck dock assignment}
\cite{lim2005transshipment} studied the cross dock and its internal transshipment problem considering time windows for supplier and customer. In this work, flow in a cross dock is constrained by warehouse capacities transportation schedules and while the objective of the problem is to minimize the total operations cost, including the inventory costs. In their next work \citep{lim2006truck}, the authors proposed a tabu search and a CPLEX-based GA for the problem they studied in \cite{lim2005transshipment}.
\cite{tsui1992optimal} Studied the truck dock assignment problem in a shipping company and proposed a bilinear model for it. In another work, \cite{Miao2009105} studied the truck dock assignment problem and proposed a MIP formulation for it, while the capacity of the cross dock over the time planning horizon is explicitly considered over the planning horizon. The authors then proposed two meta-heuristics solution algorithm, one based on tabu search and another one based on genetic algorithms. Recently, \cite{Miao2014} proposed a different MIP model for the problem, while proposing an adaptive tabu search algorithm to address the uncapacitated cases.\
\cite{chmielewski2009optimizing} studied a situation wherein, a limited buffer area is considered and unloaded pallets are placed in it, waiting for loading (at each dock door). In their version of the problem, the resources and agents required to perform this transportation, as well as the size of the buffer areas are limited. Moreover,  in their system the arrival and departure time windows are pre-defined for every truck and the objective of the problem is to, firstly, find an optimal schedule to minimize the cost of resources and secondly to minimize the waiting time for a truck receiving services.\
\cite{chmielewski2009optimizing} proposed two solution approaches, the first one, they modeled their problem as a time-discrete, multicommodity flow problem with side constraints, and to solve this mixed integer problem, they proposed a decomposition-and-column-generation approach. In their second approach, an evolutionary algorithm (EA) is proposed to identify Pareto-optimal solutions. This approach aims at minimizing the total travel distance and the total waiting time for trucks.\
\cite{dulebenets2021adaptive} proposed a mixed integer linear programming formulation for the inbound and outbound truck scheduling problem at a cross dock. \cite{dulebenets2021adaptive} considered a buffer area to help transshipment of pallets inside the cross dock for up to 24 hours. In this study, the authors have presented a mixed integer mathematical model for the inbound/outbound truck scheduling problem in cross docks and proposed a polyploid evolutionary algorithm based solution approach to solve it.\
A   case study on  how cross-docking operations can be managed more holistically in a retail distribution context in presented in \cite{buijs2016just}. In their problem description, they consider a staging/buffer area behind each dock door, where load-carriers can be temporarily placed. If used as inbound door, the staging area serves as a buffer to unload all load-carriers from an inbound trailer before they are moved through the crossdock. If used as outbound door, the staging area serves as a buffer to temporarily keep load-carriers while the consolidated outbound trailer load is fully assembled. The authors proposed a  discrete event simulation modeling order to  understand and improve the cross-docking operations. The article in particular addressed  a large grocery industry in the Netherlands.\
\cite{berghman2011optimal} presented a MIP model for a the dock assignment problem. In this study, the authors assumed that trailers need to be assigned to the dock doors for a given period of time (needed for loading/unloading activities), while the parking lot is used as a buffer zone. The internal transportation between parking lot and dock doors is performed by tractors owned by the terminal operator. A three-stage flexible flow shop problem is modeled. The first and the last stages have the same identical parallel machines. The second stage incorporates a different set of identical parallel machines. The authors examine several integer programming formulations in this work.\
A branch-and-cut algorithm is proposed in \cite{gelareh2016branch} for the truck dock assignment problem with operational time constraints. In this study, the authors also proposed a series of strengthening valid inequalities and identified some classes of facet-defining inequalities, alongside with doing a polyhedral study to improve their proposed mathematical model for the problem.

%\cite{tsui1990microcomputer} proposed a microcomputer based tool based on a bilinear program for recognition of the shipping pattern and the assignment of the dock doors.
\cite{cohen2009trailer} proposed a formulation and a new heuristic algorithm for assigning cross dock doors to trailers. \cite{deshpande2007simulating} introduced a heuristic to solve the dock assignment problem. The authors integrated the tactical level decision-making process and the operational aspects in LTL terminals to evaluate the performance of the entire system. %A case study is used to demonstrate the use of the heuristic and performance improvements.
\cite{liao2012simultaneous} studied the dock assignment problem and the sequencing problem of inbound trucks, simultaneously. They consider a multi-door cross docking operation. The objective function minimizes the total weighted tardiness, under a fixed outbound truck schedule. Six different metaheuristics are proposed, including ant colony optimization, simulated annealing, differential evolution, tabu search, and two hybrid differential-evolution algorithms. \cite{shakeri2008generic} addressed two different problems of truck scheduling and truck-to-door assignment together in a mixed integer programming model. \cite{Yu2008377} seek the best sequence scheduling for both inbound and outbound trucks in a cross duck, to minimize the total operation time when a temporary buffer storage is available to hold items temporarily at the shipping dock. In this work, assigning products to the trailers and the docking sequences of the inbound and outbound trailers are determined simultaneously. \cite{boloori2011meta} proposed a meta-heuristics algorithm to find the best sequence of inbound and outbound trailers, while their objective was to minimize the total operational time. They considered a so called temporary storage which acts as a buffer area to help managing the operation in the cross dock. \cite{arabani2010multi} deal with scheduling problem of inbound and outbound trailers in a cross docking system according to a just-in-time approach.

\cite{xi2020two} studied the cross-dock truck-scheduling problem with uncertain truck arrival and operation times. In this work, the authors introduce a concept named "conflict" and present a two-stage robust optimization model, aiming at minimizing the total operational cost as well as the number of conflicts. They then proposed a column-generation algorithm to solve their model.

\cite{ gaudioso2020lagrangian} proposed a Lagrangian heuristic algorithm for the cross-docking problem. Different products  are directly transshipped from a given set of inbound trailers to a given set of outbound ones. They assumed that the cross-docking distinguishes between the inbound and outbound dock doors to do the unloading/loading activities. It is assumed that each trailer requires a constant operation time. Scheduling the activities and designing the transshipment plan while minimizing the makespan   of the entire operation are taken into account in this work. They proposed a Lagrangian Decomposition approach (decomposed to three sub-problems) to solve their proposed ILP, while two repairing heuristics are embedded into the algorithm, to improve the calculation of both the lower and the upper bound.

\cite{ wang2019multi} present a mixed-integer nonlinear programming model and a classic linearized format of their proposed model for the multi-floor cross-dock door assignment problem  while their objective is to minimize the total material handling costs. To solve the model, they proposed a combination of multi-start, genetic-random-key and variable neighbourhood search algorithms as the diversification strategies.
% for the solution perturbation method embedded within a critical event Tabu search algorithm

\cite{ou2010scheduling} dealt with the air cargo problem and formulated the problem as a time-indexed integer programming problem. They showed that even with limited number of unloading dock doors at a terminal, the problem is quite difficult to solve. The authors proposed an exact solution procedure to determine an optimal unloading sequence of the shipments carried on each trailer, together with a Lagrangian relaxation-based heuristic for assigning the trailers to the dock doors as well as determining the trailers arrival time. Some similar models with application in the airport dock assignment problem have been studied in \cite{babic1984aircraft,ding2004new,ding2005over,oh2006dock} and \cite{lim2005airport}. \cite{agustina2010review} addresses the distribution planning problem in a cross docking network, considering transshipment possibility between the cross docks and tardiness permission for some pickups. The authors proposed a bi-objective integer programming model minimizing the total transportation and holding costs as well as the total tardiness. A heuristic procedure is proposed to construct an initial solution as well as three other metaheuristics to improve the feasible bound. \cite{kim2013gate} studied the problem of minimizing the total operational cost of the multi-cross-dock distribution network, while the total operational cost includes the transportation cost, the inventory handling cost and the penalty cost. They proposed an  adaptive genetic algorithm  and an adaptive tabu search in order to efficiently solve the problem instances.

\cite{fonseca2019hybrid} studied the truck-scheduling problem in a parallel dock cross-docking center. A two-machine flow shop scheduling  with precedence constraints modeling approach is proposed for this problem. Their objective function aims at minimizing the makespan. Later, they generalized their proposed model to the parallel-dock problem. They proposed a Lagrangian metaheuristic algorithm to solve their model using the volume algorithm to solve the dual problem. They also proposed a series of strengthening cuts to improve the dual bound obtained in every iteration.

\cite{ gelareh2020comparative} propose 8 different MIP model for the dock door assignment problem in cross-docks and alongside with three other MIP models they have reported from the literature, they undertake a comparative study and demonstrate the mathematical equivalence of all the 11 models, in order to identify the better ones, considering different properties, strengths and weaknesses.

A bi-objective MIP model is presented in \cite{ rahbari2019vehicle}  for the vehicle routing and scheduling problem with cross-docking in the context of perishable products. In this study, two robust models were developed for the situation when the travel time of outbound trailers and the freshness-life of the products were uncertain.

\cite{ monaco2020managing} proposed a MILP model. However, aiming at minimizing the completion time of the whole transhipment process, their proposed solution method is a heuristic. The main contribution of this study is to explicitly consider the transhipment flows between inbound and outbound trailers as a part of the decision problem and assume to optimise that as well. The authors proposed a Lagrangian heuristics algorithm to solve their proposed model.

\cite{Shi2013695} proposed a discrete-event simulation including an enhanced robust design technique. A multi-response optimization problem as a component of their logistics management problem has been studied. The authors aimed at designing a robust configuration for a cross-docking distribution center. Being insensitive to the disturbances of supply uncertainty and reliable in steady parts supply to downstream assembly plants are among the main focus of authors.


\cite{Buijs2014593} specified the interdependencies between different aspects of the cross-docking problem. The authors proposed a new general classification scheme for the cross-docking problem based on the inputs and outputs aspect of every research work. They also highlighted the importance of synchronization in cross-docking networks operation and described two real-life problems that were not yet addressed in the literature.

%\subsection{scheduling}
%\cite{Sadykov2012} considered the truck scheduling problem with the objective to minimize the storage usage during the product transfer inside the terminal. He showed that the problem is NP-hard and proposed a dynamic programming algorithm for a special case with fixed subsequences of incoming and outgoing trucks.
%\cite{yu2008scheduling} considered scheduling of inbound and outbound trucks in cross docking systems with temporary storage. Their objective is to find the best truck docking or scheduling sequence for both inbound and outbound trucks to minimize total operation time when a temporary storage buffer to hold items temporarily is located at the shipping dock.
%\cite{boysen2010truck} considered special truck scheduling problem arising in the (zero-inventory) cross docks of the food industry, where strict cooling requirements forbid an intermediate storage inside the terminal, so that all products are to be instantaneously loaded onto refrigerated outbound trucks. He proposed exact and heuristic algorithms.


%They considered a multi-criteria scheduling in which primary objective is to minimize earliness and tardiness simultaneously via a unified objective function. Three meta-heuristic algorithms are proposed.
%\cite{Bellanger20131109} modeled the scheduling operation as a three-stage hybrid flowshop, in which shipments and orders are represented as batches. The first stage corresponds to the receiving docks, the second stage stands for the sorting stations, and the third stage represents the shipping docks. The objective is to find a schedule that minimizes the completion time of the latest batch. They proposed several heuristic algorithms for solving instances of problem. \cite{boloori2011multi} addressed  three multi-objective algorithms including non-dominated sorting genetic algorithm-II (NSGA-II), strength Pareto evolutionary algorithm-II (SPEA-II) and sub-population genetic algorithm-II (SPGA-II) to solve the cross docking scheduling problem. \cite{zhang2010scheduling} deal with both time and space scheduling of inbound and outbound trucks at a cross dock facility under various objectives. Three different objectives in optimizing cross dock operations are presented and the justification for the use of these objectives is given.  \cite{boysen2013truck} considered truck scheduling in cross docking terminals with fixed outbound departures. They developed a heuristic algorithm for solving instances of problem.
%\end{comment}
%In layout planning, \cite{bartholdi2000reducing} used the travel cost and models of congestion at cross docks and developed a layout that minimizes labor load of work and therefore minimized the labor cost. They studied a particular case of LTL industry.\\
%\cite{stephan2011vis} carried out a comparison study of different cross dock layouts;\cite{vis2011layout} deal with the layout and control policies for cross docking operations.\\


==> mathematicalmodel.tex <==
\section{Mathematical Model}\label{sec::model}
Two models are proposed for this problem. The first one, which is a big-M model is only for demonstration purpose while the second one is the focus of this work. \\

To model the problem, the following parameters are used. \\
First of all, we define a dummy trailer '0' for the purpose of modeling. Let us define $\mathcal{J}^\circ = \mathcal{J}\cup \{0\}$. Given $T$, the planning horizon is defined by the interval $[0,T)$. Let $\delta_j$ represents the setup time required a trailer aligned to a dock door; $p_j$ represents the processing time required to serve trailer $j$ while $r_j$ and $d_j$ represent the earliest arrival and the latest departure time, respectively. We assume that %$a_0=\delta_0 = 0$,
$\delta_0 = 0$, $d_0=T$  and the first trailer to be served by every dock is this dummy trailer ('0'). Indeed, $|\mathcal{D}|<< |\mathcal{J}|$ and furthermore it is straightforward to assume that the number of "already served" trailers in every instance of the problem is no less than the number of available docks, $|\mathcal{D}|$ (unless, the instance would have an obvious solution and no effort would be needed!). For all trailers $i \in \mathcal{J}$, $f_i$ represent the penalty cost charged for every unit of the time trailer $i$ is waiting to be served, and finally, $g_i$ represents the penalty cost of not serving trailer $i$ during the current planning horizon.

\subsection {Formulation 1: Big-M model}
The following variables and parameters are introduced for this model. For a given $i$, $j$ and $d$, variable $x_{ijd}$ takes 1, if serving trailer $i$ on dock $d$ is followed by serving trailer $j$ on dock $d$, and $0$, otherwise. For a given $j$, variable $z_j$ takes value $1$, if trailer $j$ could not be served during the planning horizon and it is planned for the next day (the next planning horizon). $C_i$ represents the completion time of trailer $i$, $S_i$ stands for the time that trailer $i$ has to wait before being served, and $y_{id}$ takes $1$, if trailer $i$ is assigned to dock $d$ to be served.\\

\textbf{Dock Scheduling and Truck Sequencing (DSTS-M)}\
\begin{align}
%\small
min \:      & \sum_{i\in \mathcal{J}} f_i S_i + \sum_{j \in \mathcal{J}} g_jz_j
\label{eq:bigM:obj1}\\
            s.\:t.\:\nonumber\\
            &   \sum_{d\in \mathcal{D}}y_{jd} + z_j =1, &   \forall~ j\in\mathcal{J},\label{eq:bigM:eq1}\\
            &   \sum_{j \in \mathcal{J}^\circ, j\neq i} x_{jid} = y_{id},&    \forall~ i\in\mathcal{J},d\in\mathcal{D},\label{eq:bigM:eq2}\\
            &   \sum_{j \in \mathcal{J}^\circ, j\neq i} x_{ijd} = y_{id},&    \forall~ i\in\mathcal{J}, \forall~ d\in\mathcal{D}, \label{eq:bigM:eq3}\\
            &   C_i  + p_j + \delta_j - C_j \leq  M (1 - x_{ijd}),&    \forall~ i\in\mathcal{J}, \forall~ j\in\mathcal{J}^\circ, d\in\mathcal{D}, \label{eq:bigM:eq4}\\
            &   C_j - (r_j + p_j + \delta_j) (1 - z_j) \geq  0,&    \forall~ j\in\mathcal{J}, \label{eq:bigM:eq5}\\
            &   \sum_{j\in\mathcal{J}^\circ} ~\sum_{d\in\mathcal{D}} x_{0jd} = |\mathcal{D}|, & \label{eq:bigM:eq6}\\
            &   \sum_{j\in\mathcal{J}^\circ} ~\sum_{d\in\mathcal{D}} x_{j0d} = |\mathcal{D}|, & \label{eq:bigM:eq7}\\
			&   C_j \leq |T|-1, & \forall~ j \in \mathcal{J}\label{eq:bigM:eq8}\\
			&   S_j \geq  C_ j - (r_j + p_j + \delta_j), & \forall~  j\in \mathcal{J} \label{eq:bigM:eq9}\\
            &   x \in \{0,1\}^ {|\mathcal{J}^\circ|\times|\mathcal{J}|^\circ|\times|\mathcal{D}|}, ~            C\in \mathcal{R}^{|\mathcal{J}|}
            , y \in \{0, 1\}^{|\mathcal{J}|\times|\mathcal{D}|}, z \in \{0,1\}^ {|\mathcal{J} |}\label{eq:bigM:vars}.
\end{align}
\eqref{eq:bigM:obj1}, he objective function in this model minimizes the cost of trucks waiting to be admitted to receive services plus the penalty cost of unfulfilled services. Constraints \eqref{eq:bigM:eq1} guarantee that either a truck is allocated to a dock door to be served or should be considered as an unfulfilled service (during the current day/planning horizon). If trailer $i$ is being served by dock $d$, then it has to be scheduled to be served after (before) another trailer $j$ including the dummy trailer ($0$) as guaranteed by constraints \eqref{eq:bigM:eq2} (and \eqref{eq:bigM:eq3}) (the dummy trailer is the one that is served before and after all sequences of served trailers at every dock door). Constraints \eqref{eq:bigM:eq4} ensure that if trailer $j$ is being served after trailer $i$ on dock $d$, then it cannot be completed before the completion time of $i$, plus the docking time of $j$, plus the processing time of $j$. Constraints \eqref{eq:bigM:eq5} make sure that if trailer $j$ is served, then the completion time of this trailer cannot be less than its arrival time, plus its docking time, plus its processing time. Constraints \eqref{eq:bigM:eq6} and \eqref{eq:bigM:eq7} ensure that a trailer, which may be even the dummy trailer, follows (precedes) the dummy trailer on every dock. Constraints \eqref{eq:bigM:eq8} introduce the planning horizon. Finally, for a trailer that has already been served, constraints \eqref{eq:bigM:eq9} determine the delay between its arrival time and the time the trailer starts receiving services.

\subsection {Formulation 2: Arc-time-dock indexed model}
The following additional variables and parameters are being used. The planning horizon (that is considered as a day in this case), is divided into discrete time segments $\mathcal{T} = \{0,1,2,\dots, |T|\}$. The number of segments must not be too long or too short, however, . Variable $x_{ijdt}$ takes value $1$ if serving trailer $i$ at dock door $d$ is already finished and dock door $d$ starts serving trailer $j$ at time period $t$, $0$, otherwise. And finally, $z_j$ takes value $1$ if trailer $j$ is not served, and it takes $0$, otherwise.\\

% **********************************************************
% Formulation for the HLPVRP
% **********************************************************
\input{TimeArcIndex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{An illustrative example}
As depicted in \autoref{fig:illustrativeexample}, a solution to this problem corresponds to a network with node '0' being the source and the sink at the same time. There are $|\mathcal{D}|$ separate paths (with respect to the non-dummy trailers) starting and ending at '0'. We have considered $|\mathcal{D}|=3$, $|\mathcal{J}^\circ|=10$ and two time horizons $|\mathcal{T}|=30$ and $|\mathcal{T}|=70$. We use CPLEX 12.10, and $f_i = g_i=100,~\forall i\in \mathcal{J}$. The number of trailers and their attributes are listed in \autoref{tbl:illustrativeexample}.\\

\begin{table}
\centering
\small
\begin{tabular}{|l|l|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
Task no. &	$r_j$	& $d_j$	&  $p_j$  &	$\delta_j$\\\hline
1	&     5	    &     15	&     5	&     1\\
2	&     5	    &     20	&     5	&     1\\
3	&     5	    &     25	&     5	&     1\\
4	&     10	&     35	&     5	&     1\\
5	&     10	&     40	&     5	&     1\\
6	&     15	&     45	&     5	&     1\\
7	&     20	&     45	&     5	&     1\\
8	&     15	&     50	&     5	&     1\\
9	&     25	&     45	&     5	&     1\\
10	&     30	&     50	&     5	&     1\\
  \hline
\end{tabular}
\caption{A simple and artifice example for illustrative purpose.}
\label{tbl:illustrativeexample}
\end{table}
As one may observe in \autoref{fig:illustrativeexample}, in absence of sufficient time to serve trailers, the trailers are excluded from the day/shift service plan. In \autoref{fig::T30}, trailers 9 and 10 are left for the next day/shift service.

\begin{figure}[htb]
        \begin{subfigure}[htb]{0.48\textwidth}
                \includegraphics[width=\linewidth]{T=70}
                \caption{$T=70$}\label{fig::T70}
        \end{subfigure}%
        \begin{subfigure}[htb]{0.48\textwidth}
                \includegraphics[width=\linewidth]{T=30}
                \caption{$T=30$}\label{fig::T30}
        \end{subfigure}%
        \caption{Here is the same instance of the problem with two different horizon lengths. The shorter horizon excludes nodes 9 and 10 from the service. The actual starting time of every service for a trailer is indicated next to it.}
        \label{fig:illustrativeexample}
\end{figure}
%\begin{figure}[!ht]
%\centering
%%\includegraphics[width=0.5\textwidth]{gull}
%\input{example}
%\caption{Illustrative example with  $|\mathcal{R}|=3$, $|\mathcal{J}^\circ|=7$ and  $|\mathcal{T}|=16$.}
%\label{fig::arc-time-index}
%
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Symmetry issue}
While the model \eqref{eq:arcTimeIndex:obj1}-\eqref{eq:arcTimeIndex:vars} is already complete and solving it delivers the optimal solution, there is an issue regarding the symmetry inherent in the problem, mainly because variables $x_{i0dt},~\forall i,d,t$ do not appear in the objective function. For a given $i,d,t$, variable $x_{i0dt}$ takes 1 if $i$ is already completed and $0$ if it starts at time $t$. As this variable does not appear in the objective function, $0$ can be started sometime between the end of the service to the previous real trailer and $t=T-1$, hence multiple optimal solutions and symmetry issue. For instance, looking into \autoref{fig::T30}, one notices that the first path starts by serving $0$ serving the dummy trailer and completing its service at $t=0$. As trailer 2 arrives at $t=5$, we have $x_{0205}=1$. Trailer 2 needs a 1+5 setup and processing time and can be discharged at $t=11$ leading to $x_{25011}=1$ as trailer 5 is the one to be served the next. Trailer 5 also needs a 1+5 setup and processing time and can be discharged at $t=17$. Now, assume that the next trailer to be served is 0 and the corresponding dock door stops serving any other trailer. This means that we will have one and only one non-zero variable $x_{500*}=1$ where '*' can be any value from 17 to $T=29$, without any impact on the objective value, hence multiple solutions with the same objective value. This is an example of where symmetry occurs.\\

We can circumvent this situation and eliminate this source of symmetry by introducing constraints \eqref{eq:arcTimeIndex:symmetry} making sure that '0' will start immediately after the last real trailer being departed.

\begin{align}
            & x_{i0dt} \leq ~\sum_{l \in \mathcal{J}: ~l\neq i} ~x_{l~i~d~ t - p_i - \delta_i}         & \forall~ d \in \mathcal{D}, i \in \mathcal{J}, t \in \mathcal{T}, \label{eq:arcTimeIndex:symmetry}
\end{align}

\subsubsection{Preprocessing}
%While in the first look, the model \eqref{eq:arcTimeIndex:obj1}-\eqref{eq:arcTimeIndex:vars} may look challenging due to its number of variables, in fact, an advantage of this model is that, an important part of such variables can be eliminated in a preprocessing phase. Firstly,  variables are only introduced for the interval of arrival to the latest departure of every task and secondly, even within those intervals many options are off the table.\

An advantage of the model presented in \eqref{eq:arcTimeIndex:obj1}-\eqref{eq:arcTimeIndex:vars} is that, in fact an important number of the decision variables used in this model can be eliminated in a preprocessing phase. At the first step, variables are introduced only for the interval of the first arrival to the last departure of every task; and at the second step, even within those intervals many options are off the table. More explanations are followed.\


\begin{lem}
On every dock door, the first trailer $i\in \mathcal{J}$ must be served immediately upon its arrival. Therefore, $x_{0idt}=0, ~\forall t\geq r_i+1$.
\end{lem}

%\begin{lem}
%On every dock, no truck $i\in \mathcal{J}$ can be served before its arrival. Therefore, $x_{ijkt}=0, ~\forall i \in\mathcal{J}^0, t\leq r_i-1$.
%\end{lem}



%\begin{lem}
%In all following situations, the variable $x_{ijkt}$ can be removed from the model: 1) if $i>0,~ t>d_j$,  2) if $i>0,~ t< r_j$, 3)  if $i>0,~ t< r_i+\delta_i+p_i$, 4)  if $i>0,~  t+  \delta_j+p_j > d_j$, 5)  if $t > d_j$ or $ t< r_j$.
%\end{lem}
%
\begin{lem}
In all situations listed below, if $i \in \mathcal{J}$, variable $x_{ijdt}$ can be removed from the model: 1) if $ t > d_j$, 2) if $ t < r_j$, 3) if $t < r_i + \delta_i + p_i$, 4) if $ t +  \delta_j + p_j > d_j$.
\end{lem}

\begin{lem}
In all situations mentioned below, variable $x_{ijkt}$ can be removed from the model: 1) if $ i = 0,~ t > d_j$, 2) if $ i = 0,~ t < r_j$, 3) if $ i = 0,~ t + \delta_j + p_j > d_j$, 5) if $ i = 0, t + p_j + \delta_j > |T| - 1$.
\end{lem}

\subsection{Valid inequalities}\label{sec:valid}
Further valid inequalities can be introduced to either improve the polyhedral description or contribute to the computational performance of solvers on \eqref{eq:arcTimeIndex:eq1}-\eqref{eq:arcTimeIndex:eq61}. We will also  make use of these valid inequalities in the cutting phase of our branch-and-cut-and-price approach.

\begin{enumerate}[a)]
\item There is no 3-cycle in the order of trailers on a given dock.
\begin{align}\label{eq:valid:1}
&   \sum_{t\in \mathcal{T}}(x_{ijdt}+x_{jldt} + x_{lidt}) \leq 2, &   \forall d\in \mathcal{D},\underset{j\neq i, l\neq i, l\neq j}{\{i,j,l\}}\in \mathcal{J},
\end{align}
%\item a real truck $i\in \mathcal{J}$ must be followed (be precede) by a another truck $j\neq i\in \mathcal{J}$.
%\begin{align}
%&   \sum_{t=p_0}^{|\mathcal{T}|}\sum_{j\in {|\mathcal{J}^\circ|}}x_{ijrt} \leq \sum_{t=p_0}^{|\mathcal{T}|}\sum_{j\in {|\mathcal{J}^\circ|}}x_{jirt}, &   \forall r\in \mathcal{R}, i\in \mathcal{J},
%\end{align}
\item On the same dock door, no two real trailers can be served at the same time.
\begin{align}\label{eq:valid:2}
&   \sum_{i \in \mathcal{J}}~\sum_{j \in \mathcal{J}^\circ: ~j\neq i}~ x_{ijdt} \leq 1, &   \forall~ d \in \mathcal{D}, t \in \mathcal{T}\\
&   \sum_{i \in \mathcal{J}}~\sum_{j \in \mathcal{J}^\circ:~j \neq i}~ x_{jidt} \leq 1, &   \forall~ d \in \mathcal{D}, t \in \mathcal{T}
\end{align}
\item Two arcs in opposite directions do not appear in any feasible solution:
\begin{align}\label{eq:valid:3}
&\sum_{d \in \mathcal{D}}~\sum_{t=p_0}^{T}~ (x_{ijdt} + x_{jidt}) \leq 1,   &   \forall~ i \in \mathcal{J}, j \in \mathcal{J^\circ}, j \neq i
\end{align}


%\item The total number of variables $x_{ijrt},~ i,j\neq i \in \mathcal{J}^\circ, ~r\in\mathcal{R}, t \in \mathcal{T}$ taking 1 in any feasible solution is constrained as following:
%\begin{align}
%&\sum_{i,j\neq i \in \mathcal{J}}\sum_{r\in\mathcal{R}}\sum_{t \in \mathcal{T}}x_{ijrt} = |\mathcal{J}|,&\\
%&\sum_{i,j\neq i \in \mathcal{J}^0}\sum_{r\in\mathcal{R}}\sum_{t \in \mathcal{T}}x_{ijrt} = |\mathcal{J}|+2|\mathcal{R}|.&
%\end{align}
%\item on every rig $r$ either at some point $t\in \mathcal{T}$ a task $j\in \mathcal{J}$ is started (finished) as the first (last) task or $x_{00r0}=1$ or \eqref{eq:arcTimeIndex:eq7} (\eqref{eq:arcTimeIndex:eq8}).
%\begin{align}
%            &   \sum_{r\in \mathcal{R}}\sum_{j\in \mathcal{J}}\sum_{t\in\mathcal{T}}x_{0jrt} +x_{00r0}=1,   &                \forall r\in \mathcal{R},           \label{eq:arcTimeIndex:eq7}\\
%            &   \sum_{r\in \mathcal{R}}\sum_{j\in \mathcal{J}}\sum_{t\in\mathcal{T}}x_{j0rt} +x_{00r0}=1,   &                 \forall r\in \mathcal{R},          \label{eq:arcTimeIndex:eq8}\\
%\end{align}
%\item Every task is excused t some point in time:
%\begin{align}
%&\sum_{t\in \mathcal{T}}\sum_{i,j\in \mathcal{J}}\sum_{r\in \mathcal{R}}x_{ijrt} =1&
%\end{align}
%\item For two distinct well $i,j$ on the same machine $k$, either of them is executed before the other one:
%\begin{align}
%&\sum_{t\in \mathcal{T}}\sum_{r\in \mathcal{R}}(x_{ijrt} +x_{jirt} )=1,      &   i,j\in \mathcal{J}
%\end{align}
\end{enumerate}

%The aforementioned constraints are particularly useful when dues to some relaxation or reduced cost update in the Lagrangian relaxation or the pricing problem of column generation the cost of some variables becomes negative. There, these constraints serve to avoid too many variables  take 1 and will tighten the pricing problem/Lagrangian relaxation polytop tighter.




%\subsubsection{variable fixing by task-machine feasibility}
%As stated in the problem description, the workover rigs of larger size can serve those well of equal or smaller size while the inverse does not hold.
%
%Let  $\mathcal{R}(j)$ the represent the set of all workover rigs that can serve task $j$. The following constraint ensure the feasibility of  task assignment.
%
%\begin{align}
%&x_{ijrt} = 0&    \forall i,j \in \mathcal{J}:j\neq i,  r\notin \mathcal{R}(i) \vee r\notin \mathcal{R}(j) &
%\end{align}






%
%
%\begin{figure}
%        \begin{subfigure}[b]{0.48\textwidth}
%                \includegraphics[width=\linewidth]{T=70}
%                \caption{$T=70$}\label{fig::T70}
%        \end{subfigure}%
%        \begin{subfigure}[b]{0.48\textwidth}
%                \includegraphics[width=\linewidth]{T=30}
%                \caption{$T=30$}\label{fig::T30}
%        \end{subfigure}%
%        \caption{Modeling paradigm. The same problem instance with two different horizon length. The shorter horizon excludes nodes 9 and 10 from the day service. The starting time of every service for every truck is indicated above it.}\label{fig:example}
%\end{figure}
%
%%
%%\begin{figure}
%%\centering
%%\subfigure[$|\mathcal{T}|=70$]{%
%%\label{fig:example70}%
%%\includegraphics[width = 0.46\textwidth]{T=70}}%
%%\qquad
%%\subfigure[$|\mathcal{T}|=30$]{%
%%\label{fig:example30}%
%%\includegraphics[width = 0.46\textwidth]{T=30}}%
%%\caption{The same problem instance with two different horizon length. The shorter horizon excludes nodes 9 and 10 from the day service. The starting time of every service for every truck is indicated above it.}\label{fig:example}
%%\end{figure}
%%
%



==> numerical.tex <==
\section{Computational Experiments}\label{sec::numerical}
Due to the confidentiality, we can only report our computational results on the randomly generated instances of the problem. However, these instances are generated based on the same pattern as in the real practice instances. \\

Our computational experiments are all conducted on a machine having the following specification: Intel(R)Core(TM)i7-4770 CPU, two processors with 3.40 GHz each, and 8GB RAM. The runs are made on a 64-bit machine. The codes are written in C++ and compiled under Window 10, 64-Bit. ILOG CPLEX 12.10.0 Concert interface has been used for solving the pricing problem of the branch-and-price of the time-art-indexed formulation. 

%%%%%%%%%%%%%%%%%%% get back later 

%Some Callbacks such as \texttt{ILOUSERCUTCALLBACK}, \texttt{ILOLAZYCONSTRAINTCALLBACK} and \texttt{ILOMIPINFORCALLBACK}, were used to control, customize and influence the flow of algorithm as well as introducing custom termination criteria.\\

Our branch-and-price is an in-house efficient and engineering design code that has been developed, maintained and improved since more than a decade.\


\subsection{Instance generation} Based on real scenarios of daily operations, a discrete-event simulation model is developed, tested and validated. This discrete-event simulation model is then used to generate random instances used in this work.

In here, we are considering regional cross-docks of average size with a moderate number of dock doors, let say $20 \leq |\mathcal{D}| \leq 60$ and number of trailers $3 \times d \leq |\mathcal{J}| \leq \min\{4 \times d, 200), \forall ~ d\in \mathcal{D}$. In total, to perform this study, 236 instances were generated. The continuous time is discretized by using segments of 30 minutes. Therefore, an $8-hour$ shift corresponds to $TF=16$ and arrival times are randomly generated numbers that are following uniform distribution in interval $(0, TF\times 0.75)$. Trailers' service times are generated using uniform distribution and within interval $(\frac{tf}{8}, \frac{tf}{4})$. Likewise, docking times are generated following $U(1,3)$ and a random number $U(3,5)$ is added to those values to achieve the complete time window (which also includes the grace time). The penalty costs, $f_i$ for a unit of waiting time for trailer $i$ is generated following the uniform distribution function $U(5,10)$. The penalty cost for not serving a trailer during the current planning horizon is considered equal to $g_i = 100\times f_i$.\\



In its general form, trucks have different levels of importance with proportional monetary penalty cost if failing to fulfill their demand or for any unit of time between their arrival and start of their admission.\\

Instance names are defined following the format '$tf\_yy\_tr\_zz$' where 'yy' corresponds to the number of dock doors and 'zz' refers to the number of trailers to serve.\\

A typical temporal distribution of tasks (inbound/outbound trucks) with earliest arrival time on the left hand side and latest departure time on the right hand side of the bars is depicted in \autoref{fig:example}.

\begin{figure}[htp]
\centering
	\includegraphics[width=0.8\linewidth]{analysis}
	\caption{Temporal distribution of truck time windows for an instance with $|\mathcal{D}|=32$ and $|\mathcal{J}|=101$. The color intensity is proportional to the processing time plus docking time. Lighter color corresponds to a looser time windows and darker color corresponds to tighter ones.}
	\label{fig:example}
\end{figure}


When solving the model represented in \eqref{eq:arcTimeIndex:obj1} - \eqref{eq:arcTimeIndex:vars} (considering the compact formulation), the time limit is set to 10,800 seconds (equivalent to three hours) for solving these instances (using CPLEX 12.10). However, it is worthy to note that in some cases, solving LP at a given node of the Branch-and-Bound tree has taken longer time and therefore CPLEX did not manage to terminate its process at exactly 10,800 seconds. In such cases, what happens is that it terminates upon completion of the LP resolution at the current node of the Branch-and-Bound tree. This may result in slight deviations from the 10,800 seconds in some cases.


\subsection{Direct Solution of DSTS and DSTS-M compact formulations}

As mentioned previously, DSTS-M is a trivial mathematical model, which does not show any good computational performance mainly due to the big-M nature of the model and the naturally poor quality of the lower bound it delivers. When using this model, none of the instances of this problem, even the smallest one from among our test-bed (e.g. 20 dock doors and 60 trailers to serve) can be solved to optimality within the 3 hours time frame using a modern commercial solver, e.g. CPLEX. \\
%For an example of the smallest instance of the problem within a time-frame of 3 hours for 20 docks and 60 trucks, we obtain a feasible solution with the objective function's value 1406.00 and the best dual bound 1988.00 while the optimal objective value for this instance is 970.00. Moreover, to achieve this poor results CPLEX had to process 417172 nodes. On one hand, it means that the LPs are rather easy to solve (for CPLEX) but on the other hand, they do not produce meaningful information allowing improvement of the dual bound or helping the heuristic processes inside CPLEX to generate better feasible solutions (primal bound). We therefore concentrate our analysis on the DSTS model. \\

From among the valid inequalities presented in \autoref{sec:valid}, only a very few of them (among \eqref{eq:valid:1}) seemed to be violated and could be added to the model at some fractional nodes. Yet, the number of such separated cuts were so few that the computational overhead did not pay off. We therefore, abandoned the idea of a Branch-and-Cut and resorted to a direct solver using CPLEX. Thus, we refer to this as a direct application of CPLEX for solving instances of this problem.\\

In \autoref{tbl:directCplex}, the first column refers to the instances' name while the second one ('Obj. Val.') represents objective value upon termination of CPLEX. In comuln 3, ('\#Nodes'), The number of nodes processed before termination of the solver is reported, while the status of the solver upon termination is reported in the column under the term ('Status'). The computational time ('CPUTime') spent to solve an instance, for every instance is represented in the subsequent column. The last column in this table reports the time the heuristic algorithm spends to solve the instance of the problem. \\

\begin{footnotesize}
    \begin{longtable}{lccccccccccc}
    \caption{Computational experiments of solving real-life-size instances of of the problem, using CPLEX.}\label{tbl:directCplex} \\
\specialrule{.2em}{.1em}{.1em}
\input{resCplex}
%\specialrule{.2em}{.1em}{.1em}
     \end{longtable}
\end{footnotesize}


As it can be observed in \autoref{tbl:directCplex}, for very small size instances of 20-26 dock doors and 60-100 trailers within a time limit of 3 hours, only 6 instances were solved to optimality. In this table, whenever no optimal solution is at hand, the status of the solver upon termination as well as the MIP relative gap (theration of the distance between the best known feasible solution and the best known dual bound) is reported in parenthesis next to it. The reported gaps are relatively high. For three instances (in \textbf{bold}) the objective values correspond to that of the optimal solution but the optimality could not be proven within 3 hours. The number of branch-and-bound nodes processed remains reasonable indicating that for very few instances, LP could be resolved during the time limit (10,800 seconds), indicating that even the LP reoptimization becomes a challenge.\\

Later, we have also lifted this time limit hoping for some improvement and maybe some additional information, but not much could be achieved into those outputs.\




\subsection{Branch-and-price solution approach}
In \autoref{tbl:realistic}, the first column of the table refers to the instances' name. Remaining columns are: the objective value, the number of nodes which are processed in the Branch-and-Bound tree at the master problem level, the status of the last pricing problem before termination of the whole process, the computational time, the number of generated columns during the solution procedure (apart from the initial column), the number of calls to the pricing problem and finally the service level ratio (percentage of served trailers amongst all).\\

An initial column is always added, which is generated using the heuristic seen in \autoref{heurs} allowing a warm-start of the master problem. Thus, we always have a feasible restricted master problem. When solving the pricing problem, emphasis is put on quick bound improvement (breadth-first search) and the subproblem solution is terminated upon meeting any of these criteria: 1)3600 seconds passed and a solution to the problem is found that has negative objective value, 2) 3$\times$ 3,600 seconds (3 hours) has been elapsed on solving the pricing problem while the objective value still remains at $0$. As CPLEX is being used to solve the subproblem, each time the solution process of the pricing problem starts from where the previous one is terminated. That is, CPLEX is already aware of some feasible solutions as its solution pool has not been emptied. \\

In our initial computational experiments, we have been generating one column per iteration and that caused more number of iterations and columns leading to longer computational times. In fact, our observations out of an extensive initial computational experiments, confirmed that after each iteration the pricing problem resolution was becoming significantly less efficient. Therefore, we decided to warm start each pricing re-solve from where it stopped in the previous iteration, this has improved the solution but not very significantly. The last resort was to add all columns to the master problem, with negative objective value for the pricing problem. \\

In the same initial experiments, we have also examined efficiency of the pricing problem solution by separating cuts from among those aforementioned valid inequalities, but it revealed that the overhead of doing so is often beyond the achieved efficiency  and therefore, does not pay off. We therefore, did not separate any of those cuts when solving the pricing problem. \



\begin{footnotesize}
    \begin{longtable}{lccccccccccc}
    \caption{Computational experiments of solving real-life-size instances of the problem using the branch-and-price algorithm.}\label{tbl:realistic} \\
\specialrule{.2em}{.1em}{.1em}
\input{Largest}
%\specialrule{.2em}{.1em}{.1em}
     \end{longtable}
\end{footnotesize}

From among the initial 236 instances, given time limits and setups, for 191 instances, the optimal solution was proved, using the proposed Branch-and-Price solution algorithm. In 44 cases the last pricing problem has been terminated with an objective value equal to 0 while the optimality has not been proven. In one case, CPLEX encountered memory issue ('FailFeasNoTree') while it has already found at least one integer feasible solutions.\\

For all above instances, in situations where the last pricing problem turned to be not-optimal (when the solve procedure terminated by 'AbordUser'), for all those cases, we report the absolute gap between the best incumbent and the best lower (dual) bound. There are situations where these two values coincide but CPLEX has been still busy doing something and thus, not been terminated.\\

As a summary, one observes that the approach is capable of dealing with real-life-size instances in a reasonable time. Moreover, the number of calls to the pricing problem remains below 4, also the number of added columns that remains is reasonably very few (never gets even close to 100 columns).  \\





In \autoref{tbl:realistic}, we have divided the table into blocks corresponding to every value of $d\in\mathcal{D}$. When looking at the last column, one observes that for every $d\in\mathcal{D}$ the ratio of the served trailers to the total number of them decreases as the number of trailers increases. \autoref{fig:ServedtoTotal} depicts the trend of this ratio for the instances indexed by the rows in \autoref{tbl:realistic}.




\begin{figure}
  \centering
  \includegraphics[width=0.6\textwidth]{ServedtoTotal.eps}
  \caption{The ratio of served trailers to the number of inbound trucks.}\label{fig:ServedtoTotal}
\end{figure}



\subsection{VNS-like method}
The set-up for the VNS-like algorithm follows: We terminate the whole process when $\frac{d_*}{\mathbf{T^{t}}}< \epsilon = 0.05$ and $N^{max_{NonI}^{iter}}> |J|\times |D|$. The transition matrix has been initialized with random values.\\

Since the nature of this algorithm is non-deterministic, we have run every instance 5 times and achieved the same solution at every single case. The variance in computational time of the 5 trials remained less than 2 percent of the best-known feasible solution. Our extensive initial experiments confirmed that choice of method delivering the initial solution (see \autoref{Initial-DSTS}) does not play any significant role in improving the quality of the obtained solutions or reducing the computational time required to conduct the overall solution algorithm.   \\

The computational time has never exceeds 900 seconds (equivalent to 15 minutes) and the best found feasible solution coincided with the one reported by the Branch-and-Price solution approach (reported in \autoref{tbl:realistic}). \\








==> problemdescription.tex <==
\section{Problem Description}\label{sec::problemdescription}


The problem description follows: \\


\emph{Assume $\mathcal{J}=\{1,\dots,N\}$ represents a set of trucks pulling (outbound and/or inbound) trailers, and $\mathcal{D}=\{1,\dots,D\}$ be a set of bi-functional dock doors of a cross-dock (to serve loading and/or unloading trailers). For every truck $j\in \mathcal{J}$ an arrival time $r_j$ is given as well as a strict latest departure time $d_j$. Based on expert knowledge, we assume no perturbation for arrival times however, the departure time of every truck needs to be respected following the internal operations. If the latest departure time is missed (the internal required processing time is longer than $d_j - r_j$, then the truck will have to be scheduled for the next day departure). For every truck $j\in \mathcal{J}$ given a docking time $\delta_j$, which is the time required for the operation of aligning the given trailer in front of a dock door, as well as the setups time required by both the truck and the dock door to start the loading/unloading operation. Moreover, a processing time $p_j$ (unit of time intervals) is given which is, for every truck $j\in \mathcal{J}$, required to load/unload the corresponding trailer. In its general manner, every trailer $j\in \mathcal{J}$ may belong to one or several clients and may carry similar or different cargo with different levels of sensitivity that can be interpreted as penalty cost, $f_j$, for every unit of waiting time for a trailer, before being admitted to receive services. Moreover, a penalty cost $g_j$ is considered for the situation when trailer $j$ is not served at all. We tend to minimize the waiting time of every single truck in a way that it leaves the soonest possible, also to minimize the (weighted) penalty charge of delayed or missed trucks in the daily planning of a cross-docks. }\\

In this problem description, based on experts' knowledge no capacity constraint is imposed on the problem.% as we considered that there exists a sufficient temporal stacking space within the cross-dock without causing any sort of operational inefficiencies.


==> resCplex.tex <==
Instance	& Obj. Val.	& \#Nodes	&Status	&CPUTime (sec.)	\\
\specialrule{.2em}{.1em}{.1em}
tf\_20\_tr\_60&	970.00&	8467&	Optimal&	4301.80\\
tf\_ 20\_tr\_65&	3312.00&	0&	Optimal&	24.88\\
tf\_20\_tr\_70&	1686.00&	9281&	{\scriptsize Feasible
 (58.00\%)}&	\texttt{timeLim}\\
tf\_20\_tr\_75&	3944.00&	11073&	{\scriptsize Feasible
 (31.00\%)}&	\texttt{timeLim}\\
tf\_20\_tr\_80&	5075.00&	5488&	{\scriptsize Feasible
 (10.00\%)}&	\texttt{timeLim}\\
tf\_20\_tr\_85&	8762.00&	3299&	{\scriptsize Feasible
 (42.00\%)}&	\texttt{timeLim}\\
tf\_20\_tr\_90&	12573.00&	1913&	{\scriptsize Feasible
 (34.00\%)}&	\texttt{timeLim}\\
tf\_20\_tr\_95&	14897.00&	1947&	{\scriptsize Feasible
 (19.00\%)}&	\texttt{timeLim}\\
tf\_20\_tr\_100&	16027.00&	1689&	{\scriptsize Feasible
 (32.00\%)}&	\texttt{timeLim}\\
 \hline
tf\_22\_tr\_66&	2810.00&	0&	Optimal&	36.79\\
tf\_22\_tr\_71&	636.00&	101404&	Optimal&	6755.52\\
tf\_22\_tr\_76&	\textbf{4651.00}&	15728&	{\scriptsize Feasible
 (6.00\%)}&	\texttt{timeLim}\\
tf\_22\_tr\_81&	\textbf{4328.00}&	9035&	{\scriptsize Feasible
 (13.00\%)}&	\texttt{timeLim}\\
tf\_22\_tr\_86&	7197.00&	5325&	{\scriptsize Feasible
 (25.00\%)}&	\texttt{timeLim}\\
tf\_22\_tr\_91&	\textbf{11550.00}&	5930&	{\scriptsize Feasible
 (4.00\%)}&	\texttt{timeLim}\\
tf\_22\_tr\_96&	12124.00&	2014&	{\scriptsize Feasible
 (44.00\%)}&	\texttt{timeLim}\\
tf\_22\_tr\_101&	15236.00&	2038&	{\scriptsize Feasible
 (34.00\%)}&	\texttt{timeLim}\\
tf\_22\_tr\_106&	15208.00&	1030&	{\scriptsize Feasible
 (33.00\%)}&	\texttt{timeLim} \\
 \hline
tf\_24\_tr\_72&	2103.00&	20607&	Optimal&	9529.55\\
tf\_24\_tr\_77&	2995.00&	7128&	Optimal&	9399.61\\
tf\_24\_tr\_82&	2494.00&	4124&	{\scriptsize Feasible
 (3.00\%)}&	\texttt{timeLim} \\
tf\_24\_tr\_87&	3220.00&	2246&	{\scriptsize Feasible
 (62.00\%)}&	\texttt{timeLim}\\
tf\_24\_tr\_92&	6110.00&	1815&	{\scriptsize Feasible
 (34.00\%)}&	\texttt{timeLim}\\
tf\_24\_tr\_97&	6871.00&	2294&	{\scriptsize Feasible
 (10.00\%)}&	\texttt{timeLim}\\
 tf\_24\_tr\_102&	10952.00&	1912&	{\scriptsize Feasible
 (10.00\%)}&	\texttt{timeLim}\\
%tf\_24\_tr\_107&	0.00&	0&	Optimal&	0.00\\ 

==> table1.tex <==
\begin{landscape}
    \footnotesize
    \begin{center}
    \begin{longtable}{|l|c|c|c|c|c|c|c|}
\caption{Best solution and execution time results by the two solutions. } \label{tab:Principal} \\
    \hline
    Instance Name & \# Wells & \# WR & Init. Obj. & Best Obj. (GIHH) & CPU Time (GIHH) & Best Obj. L.M. & CPU Time  L.M. \\
\hline
    %\midrule
    Instance\_8\_3.pb & 8     & 3     & 136   & 92    & 5.277 & 92    & 4.539 \\
    Instance\_10\_3.pb & 10    & 3     & 25208 & 17074 & 4.901 & 15592 & 4.798 \\
    Instance\_15\_3.pb & 15    & 3     & 56549 & 24179 & 4.907 & 24179 & 4.293 \\
    Instance\_15\_5.pb & 15    & 5     & 32644 & 19643 & 4.772 & 17092 & 4.562 \\
    Instance\_20\_3.pb & 20    & 3     & 131288 & 63177 & 5.424 & 63177 & 4.451 \\
    Instance\_20\_5.pb & 20    & 5     & 64326 & 40448 & 5.155 & 32352 & 4.114 \\
    Instance\_25\_3.pb & 25    & 3     & 230457 & 119279 & 4.926 & 119715 & 3.698 \\
    Instance\_25\_5.pb & 25    & 5     & 138700 & 69572 & 6.284 & 74327 & 3.623 \\
    Instance\_25\_7.pb & 25    & 7     & 89556 & 52224 & 5.229 & 42565 & 3.883 \\
    Instance\_30\_3.pb & 30    & 3     & 367449 & 132035 & 5.213 & 124934 & 3.662 \\
    Instance\_30\_5.pb & 30    & 5     & 207032 & 86271 & 5.899 & 84813 & 3.808 \\
    Instance\_30\_7.pb & 30    & 7     & 116485 & 66798 & 5.208 & 64913 & 3.899 \\
    Instance\_35\_3.pb & 35    & 3     & 570353 & 156471 & 5.113 & 152520 & 3.373 \\
    Instance\_35\_5.pb & 35    & 5     & 262129 & 117794 & 4.648 & 127175 & 3.612 \\
    Instance\_35\_7.pb & 35    & 7     & 185168 & 88108 & 5.227 & 78595 & 3.683 \\
    Instance\_50\_5.pb & 50    & 5     & 626882 & 227501 & 4.853 & 196916 & 6.887 \\
    Instance\_50\_7.pb & 50    & 7     & 413490 & 168665 & 5.359 & 176627 & 7.085 \\
    Instance\_50\_9.pb & 50    & 9     & 297819 & 135071 & 5.245 & 133151 & 7.002 \\
    Instance\_50\_10.pb & 50    & 10    & 289527 & 152912 & 5.034 & 145656 & 6.983 \\
    Instance\_75\_7.pb & 75    & 7     & 936822 & 378687 & 9.797 & 387174 & 6.369 \\
    Instance\_75\_9.pb & 75    & 9     & 677938 & 308775 & 10.959 & 301691 & 6.579 \\
    Instance\_75\_10.pb & 75    & 10    & 662634 & 302610 & 10.126 & 302336 & 6.745 \\
    Instance\_100\_7.pb & 100   & 7     & 5628206 & 1505768 & 10.756 & 1460573 & 6.304 \\
    Instance\_100\_9.pb & 100   & 9     & 4818597 & 1700178 & 10.796 & 1653207 & 6.381 \\
    Instance\_100\_10.pb & 100   & 10    & 3763364 & 1558833 & 11.150 & 1472270 & 6.387 \\
    Instance\_100\_12.pb & 100   & 12    & 3301954 & 1277372 & 10.729 & 1125684 & 6.483 \\
    Instance\_125\_7.pb & 125   & 7     & 17942188 & 3976275 & 9.722 & 4113369 & 6.343 \\
    Instance\_125\_10.pb & 125   & 10    & 14217667 & 4054434 & 10.360 & 3883325 & 6.280 \\
    Instance\_125\_12.pb & 125   & 12    & 12797731 & 4073711 & 10.066 & 3959405 & 6.296 \\
    Instance\_150\_7.pb & 150   & 7     & 31561876 & 6061352 & 10.153 & 5689447 & 6.297 \\
    Instance\_150\_10.pb & 150   & 10    & 24621016 & 6381947 & 10.033 & 6381464 & 6.323 \\
    Instance\_150\_12.pb & 150   & 12    & 20818808 & 5778118 & 9.809 & 5743722 & 6.209 \\
    Instance\_175\_7.pb & 175   & 7     & 72747008 & 13040327 & 10.393 & 12664936 & 6.445 \\
    Instance\_175\_10.pb & 175   & 10    & 59779656 & 15010189 & 9.760 & 15747698 & 6.099 \\
    Instance\_175\_12.pb & 175   & 12    & 52505040 & 13868167 & 9.746 & 14298780 & 6.332 \\
    Instance\_200\_7.pb & 200   & 7     & 94706824 & 14806276 & 10.477 & 14140791 & 6.236 \\
    Instance\_200\_10.pb & 200   & 10    & 78842104 & 19800238 & 9.816 & 18930664 & 6.346 \\
    Instance\_200\_12.pb & 200   & 12    & 70074008 & 15302376 & 9.973 & 14553232 & 6.358 \\
\hline
     \end{longtable}
     \end{center}
     \end{landscape}


==> table2.tex <==
\begin{landscape}
    \footnotesize
    \begin{center}
    \begin{longtable}{|l|c|c|c|c|c|c|c|}
\caption{Number of heuristic visits by instance using GIHH. } \label{tab:VisitsGIHH} \\
    \hline
    Instance Name & Constructive & Order Improvement & Mutation & CrossOver & Intelligent Add/Delete & Reconstructive \\
\hline
     {Instance\_8\_3.pb} & {428} & {1377} & {337} & {645} & {308} & {329} \\
    {Instance\_10\_3.pb} & {280} & {1294} & {319} & {655} & {336} & {358} \\
    {Instance\_15\_3.pb} & {418} & {1325} & {302} & {596} & {294} & {329} \\
    {Instance\_15\_5.pb} & {297} & {1266} & {331} & {659} & {328} & {310} \\
    {Instance\_20\_3.pb} & {306} & {1358} & {390} & {720} & {330} & {346} \\
    {Instance\_20\_5.pb} & {275} & {1292} & {378} & {694} & {316} & {325} \\
    {Instance\_25\_3.pb} & {457} & {2519} & {625} & {1383} & {758} & {583} \\
    {Instance\_25\_5.pb} & {291} & {2453} & {255} & {545} & {290} & {1814} \\
    {Instance\_25\_7.pb} & {293} & {1178} & {225} & {445} & {220} & {479} \\
    {Instance\_30\_3.pb} & {231} & {2553} & {231} & {1299} & {1068} & {268} \\
    {Instance\_30\_5.pb} & {215} & {2106} & {1511} & {1738} & {227} & {252} \\
    {Instance\_30\_7.pb} & {265} & {1248} & {269} & {534} & {265} & {446} \\
    {Instance\_35\_3.pb} & {253} & {1341} & {348} & {570} & {222} & {534} \\
    {Instance\_35\_5.pb} & {274} & {1262} & {304} & {625} & {321} & {344} \\
    {Instance\_35\_7.pb} & {322} & {1435} & {339} & {614} & {275} & {395} \\
    {Instance\_50\_5.pb} & {558} & {1070} & {236} & {463} & {227} & {287} \\
    {Instance\_50\_7.pb} & {319} & {1341} & {291} & {589} & {298} & {341} \\
    {Instance\_50\_9.pb} & {297} & {1099} & {237} & {492} & {255} & {316} \\
    {Instance\_50\_10.pb} & {233} & {1092} & {291} & {567} & {276} & {279} \\
    {Instance\_75\_7.pb} & {363} & {1510} & {373} & {771} & {398} & {368} \\
    {Instance\_75\_9.pb} & {381} & {3370} & {427} & {758} & {331} & {2632} \\
    {Instance\_75\_10.pb} & {319} & {1623} & {411} & {788} & {377} & {535} \\
    {Instance\_100\_7.pb} & {217} & {4112} & {429} & {2094} & {1665} & {514} \\
    {Instance\_100\_9.pb} & {252} & {3439} & {244} & {1740} & {1496} & {297} \\
    {Instance\_100\_10.pb} & {283} & {3757} & {259} & {1892} & {1633} & {321} \\
    {Instance\_100\_12.pb} & {258} & {3151} & {2552} & {2746} & {194} & {268} \\
    {Instance\_125\_7.pb} & {299} & {1275} & {276} & {547} & {271} & {345} \\
    {Instance\_125\_10.pb} & {288} & {1154} & {321} & {562} & {241} & {355} \\
    {Instance\_125\_12.pb} & {287} & {1109} & {254} & {522} & {268} & {316} \\
    {Instance\_150\_7.pb} & {236} & {2138} & {248} & {1113} & {865} & {266} \\
    {Instance\_150\_10.pb} & {247} & {1109} & {251} & {544} & {293} & {286} \\
    {Instance\_150\_12.pb} & {251} & {1019} & {263} & {516} & {253} & {261} \\
    {Instance\_175\_7.pb} & {192} & {1963} & {219} & {1021} & {802} & {225} \\
    {Instance\_175\_10.pb} & {178} & {857} & {212} & {395} & {183} & {273} \\
    {Instance\_175\_12.pb} & {231} & {968} & {248} & {492} & {244} & {252} \\
    {Instance\_200\_7.pb} & {173} & {1561} & {135} & {792} & {657} & {195} \\
    {Instance\_200\_10.pb} & {208} & {875} & {231} & {442} & {211} & {248} \\
    {Instance\_200\_12.pb} & {189} & {827} & {219} & {418} & {199} & {238} \\
\hline
     \end{longtable}
     \end{center}
     \end{landscape}


==> table3.tex <==
\begin{landscape}
    \footnotesize
    \begin{center}
    \begin{longtable}{|l|c|c|c|c|c|c|c|}
\caption{Number of heuristic visits by instance using our own learning method. } \label{tab:VisitsOwn} \\
    \hline
    Instance Name & Constructive & Order Improvement & Mutation & CrossOver & Intelligent Add/Delete & Reconstructive\\
\hline
    {Instance\_8\_3.pb} & {3873} & {22013} & {4779} & {9394} & {4666} & {4768} \\
    {Instance\_10\_3.pb} & {3799} & {21033} & {4528} & {8996} & {4505} & {4458} \\
    {Instance\_15\_3.pb} & {2886} & {15984} & {3395} & {6810} & {3493} & {3396} \\
    {Instance\_15\_5.pb} & {2791} & {16001} & {3422} & {6789} & {3395} & {3514} \\
    {Instance\_20\_3.pb} & {2416} & {13676} & {2967} & {5906} & {2967} & {2888} \\
    {Instance\_20\_5.pb} & {2337} & {13389} & {2839} & {5782} & {2928} & {2852} \\
    {Instance\_25\_3.pb} & {1916} & {10661} & {2331} & {4551} & {2297} & {2255} \\
    {Instance\_25\_5.pb} & {1888} & {10770} & {2316} & {4616} & {2261} & {2343} \\
    {Instance\_25\_7.pb} & {1773} & {10156} & {2156} & {4408} & {2149} & {2209} \\
    {Instance\_30\_3.pb} & {1642} & {9343} & {1983} & {4024} & {2045} & {1945} \\
    {Instance\_30\_5.pb} & {1726} & {9635} & {2096} & {4147} & {2058} & {2074} \\
    {Instance\_30\_7.pb} & {1565} & {8994} & {1944} & {3851} & {1938} & {1922} \\
    {Instance\_35\_3.pb} & {1348} & {7218} & {1563} & {3076} & {1515} & {1553} \\
    {Instance\_35\_5.pb} & {1450} & {8098} & {1749} & {3489} & {1776} & {1660} \\
    {Instance\_35\_7.pb} & {1496} & {8267} & {1843} & {3538} & {1747} & {1782} \\
    {Instance\_50\_5.pb} & {2111} & {11530} & {2397} & {5023} & {2445} & {2417} \\
    {Instance\_50\_7.pb} & {2137} & {11550} & {2439} & {4948} & {2469} & {2491} \\
    {Instance\_50\_9.pb} & {1962} & {10965} & {2378} & {4710} & {2378} & {2315} \\
    {Instance\_50\_10.pb} & {2006} & {11430} & {2492} & {4912} & {2488} & {2392} \\
    {Instance\_75\_7.pb} & {1246} & {7070} & {1490} & {3108} & {1504} & {1447} \\
    {Instance\_75\_9.pb} & {1325} & {7277} & {1579} & {3058} & {1526} & {1594} \\
    {Instance\_75\_10.pb} & {1445} & {7657} & {1683} & {3206} & {1595} & {1696} \\
    {Instance\_100\_7.pb} & {823} & {4699} & {944} & {2028} & {1056} & {1002} \\
    {Instance\_100\_9.pb} & {909} & {5166} & {1093} & {2196} & {1110} & {1135} \\
    {Instance\_100\_10.pb} & {855} & {5096} & {1091} & {2185} & {1071} & {1156} \\
    {Instance\_100\_12.pb} & {882} & {4916} & {983} & {2168} & {1028} & {1041} \\
    {Instance\_125\_7.pb} & {620} & {3534} & {766} & {1551} & {735} & {761} \\
    {Instance\_125\_10.pb} & {642} & {3575} & {773} & {1513} & {761} & {807} \\
    {Instance\_125\_12.pb} & {599} & {3239} & {692} & {1376} & {720} & {659} \\
    {Instance\_150\_7.pb} & {404} & {2386} & {495} & {1048} & {507} & {502} \\
    {Instance\_150\_10.pb} & {446} & {2674} & {567} & {1151} & {581} & {577} \\
    {Instance\_150\_12.pb} & {478} & {2611} & {513} & {1102} & {577} & {573} \\
    {Instance\_175\_7.pb} & {341} & {1892} & {423} & {827} & {417} & {359} \\
    {Instance\_175\_10.pb} & {341} & {1970} & {423} & {836} & {417} & {436} \\
    {Instance\_175\_12.pb} & {385} & {2008} & {435} & {838} & {423} & {435} \\
    {Instance\_200\_7.pb} & {262} & {1393} & {307} & {597} & {305} & {291} \\
    {Instance\_200\_10.pb} & {280} & {1560} & {323} & {671} & {328} & {342} \\
    {Instance\_200\_12.pb} & {257} & {1418} & {293} & {582} & {303} & {332} \\


\hline
     \end{longtable}
     \end{center}
     \end{landscape}


==> table4.tex <==
\begin{landscape}
    \footnotesize
    \begin{center}
    \begin{longtable}{|l|c|c|c|c|c|c|c|}
\caption{Percentage of heuristic time consuming by instance using GIHH. } \label{tab:TimeGIHH} \\
    \hline
    Instance Name & Constructive & Improvement & Mutation & CrossOver & Intelligent Add/Delete & Reconstructive \\
\hline
 {Instance\_8\_3.pb} & 5.556 & 50.000 & 16.667 & 16.667 & 11.111 & 0.000 \\
    {Instance\_10\_3.pb} & 10.000 & 40.000 & 0.000 & 10.000 & 10.000 & 30.000 \\
    {Instance\_15\_3.pb} & 0.000 & 61.538 & 15.385 & 7.692 & 15.385 & 0.000 \\
    {Instance\_15\_5.pb} & 29.412 & 29.412 & 5.882 & 11.765 & 11.765 & 11.765 \\
    {Instance\_20\_3.pb} & 3.571 & 85.714 & 0.000 & 0.000 & 10.714 & 0.000 \\
    {Instance\_20\_5.pb} & 5.000 & 60.000 & 10.000 & 0.000 & 15.000 & 10.000 \\
    {Instance\_25\_3.pb} & 10.145 & 75.362 & 1.449 & 1.449 & 4.348 & 7.246 \\
    {Instance\_25\_5.pb} & 9.615 & 63.462 & 1.923 & 3.846 & 5.769 & 15.385 \\
    {Instance\_25\_7.pb} & 25.000 & 53.571 & 3.571 & 3.571 & 7.143 & 7.143 \\
    {Instance\_30\_3.pb} & 6.250 & 85.000 & 0.000 & 2.500 & 1.250 & 5.000 \\
    {Instance\_30\_5.pb} & 8.571 & 75.714 & 4.286 & 4.286 & 4.286 & 2.857 \\
    {Instance\_30\_7.pb} & 5.882 & 64.706 & 2.941 & 2.941 & 8.824 & 14.706 \\
    {Instance\_35\_3.pb} & 12.698 & 68.254 & 1.587 & 1.587 & 4.762 & 11.111 \\
    {Instance\_35\_5.pb} & 10.714 & 78.571 & 0.000 & 3.571 & 3.571 & 3.571 \\
    {Instance\_35\_7.pb} & 27.273 & 54.545 & 2.273 & 2.273 & 4.545 & 9.091 \\
    {Instance\_50\_5.pb} & 34.694 & 58.163 & 2.041 & 0.000 & 1.020 & 4.082 \\
    {Instance\_50\_7.pb} & 21.839 & 65.517 & 1.149 & 3.448 & 2.299 & 5.747 \\
    {Instance\_50\_9.pb} & 28.571 & 61.429 & 0.000 & 0.000 & 4.286 & 5.714 \\
    {Instance\_50\_10.pb} & 28.070 & 64.912 & 0.000 & 1.754 & 1.754 & 3.509 \\
    {Instance\_75\_7.pb} & 29.911 & 63.393 & 0.000 & 0.893 & 4.018 & 1.786 \\
    {Instance\_75\_9.pb} & 17.211 & 76.253 & 0.000 & 0.000 & 1.089 & 5.447 \\
    {Instance\_75\_10.pb} & 27.049 & 65.164 & 0.820 & 0.820 & 3.279 & 2.869 \\
    {Instance\_100\_7.pb} & 7.909 & 87.170 & 0.176 & 0.351 & 3.076 & 1.318 \\
    {Instance\_100\_9.pb} & 13.226 & 83.066 & 0.000 & 0.742 & 2.225 & 0.742 \\
    {Instance\_100\_10.pb} & 13.453 & 80.045 & 0.224 & 0.448 & 4.933 & 0.897 \\
    {Instance\_100\_12.pb} & 15.745 & 81.135 & 0.567 & 0.709 & 0.709 & 1.135 \\
    {Instance\_125\_7.pb} & 27.831 & 68.554 & 0.241 & 0.000 & 1.084 & 2.289 \\
    {Instance\_125\_10.pb} & 32.806 & 64.029 & 0.000 & 0.144 & 1.295 & 1.727 \\
    {Instance\_125\_12.pb} & 38.693 & 58.459 & 0.000 & 0.168 & 1.675 & 1.005 \\
    {Instance\_150\_7.pb} & 16.295 & 80.747 & 0.000 & 0.208 & 2.180 & 0.571 \\
    {Instance\_150\_10.pb} & 31.628 & 66.180 & 0.313 & 0.209 & 0.939 & 0.731 \\
    {Instance\_150\_12.pb} & 33.845 & 63.701 & 0.000 & 0.102 & 1.431 & 0.920 \\
    {Instance\_175\_7.pb} & 14.712 & 82.935 & 0.000 & 0.075 & 1.718 & 0.560 \\
    {Instance\_175\_10.pb} & 31.714 & 66.269 & 0.000 & 0.092 & 0.917 & 1.008 \\
    {Instance\_175\_12.pb} & 34.694 & 63.815 & 0.078 & 0.157 & 0.785 & 0.471 \\
    {Instance\_200\_7.pb} & 16.811 & 80.179 & 0.000 & 0.032 & 2.241 & 0.736 \\
    {Instance\_200\_10.pb} & 34.076 & 64.457 & 0.000 & 0.059 & 0.469 & 0.938 \\
    {Instance\_200\_12.pb} & 32.173 & 65.966 & 0.000 & 0.000 & 0.900 & 0.960 \\

\hline
     \end{longtable}
     \end{center}
     \end{landscape}


==> table5.tex <==
\begin{landscape}
    \footnotesize
    \begin{center}
    \begin{longtable}{|l|c|c|c|c|c|c|c|}
\caption{Percentage of heuristic time consuming by instance using Our Own Learning Method. } \label{tab:TimeOwn} \\
    \hline
    Instance Name & Constructive & Improvement & Mutation & CrossOver & Intelligent Add/Delete & Reconstructive \\
\hline
    %\midrule
    {Instance\_8\_3.pb} & 0.774 & 5.073 & 0.258 & 0.516 & 92.003 & 1.376 \\
    {Instance\_10\_3.pb} & 0.471 & 4.870 & 0.314 & 0.628 & 92.930 & 0.786 \\
    {Instance\_15\_3.pb} & 1.040 & 7.152 & 0.195 & 0.650 & 89.857 & 1.105 \\
    {Instance\_15\_5.pb} & 0.889 & 5.400 & 0.137 & 0.410 & 92.755 & 0.410 \\
    {Instance\_20\_3.pb} & 1.152 & 9.218 & 0.243 & 0.121 & 88.114 & 1.152 \\
    {Instance\_20\_5.pb} & 1.512 & 6.171 & 0.060 & 0.181 & 91.531 & 0.544 \\
    {Instance\_25\_3.pb} & 1.478 & 12.707 & 0.236 & 0.118 & 84.574 & 0.887 \\
    {Instance\_25\_5.pb} & 1.633 & 7.055 & 0.058 & 0.058 & 90.262 & 0.933 \\
    {Instance\_25\_7.pb} & 1.711 & 6.357 & 0.244 & 0.183 & 91.137 & 0.367 \\
    {Instance\_30\_3.pb} & 1.946 & 13.892 & 0.108 & 0.162 & 82.811 & 1.081 \\
    {Instance\_30\_5.pb} & 2.429 & 9.322 & 0.169 & 0.339 & 87.119 & 0.621 \\
    {Instance\_30\_7.pb} & 1.730 & 7.310 & 0.112 & 0.223 & 90.011 & 0.614 \\
    {Instance\_35\_3.pb} & 2.035 & 17.568 & 0.161 & 0.107 & 78.522 & 1.607 \\
    {Instance\_35\_5.pb} & 2.231 & 10.990 & 0.000 & 0.490 & 85.909 & 0.381 \\
    {Instance\_35\_7.pb} & 3.333 & 10.000 & 0.111 & 0.167 & 85.611 & 0.778 \\
    {Instance\_50\_5.pb} & 3.527 & 16.196 & 0.052 & 0.052 & 79.441 & 0.731 \\
    {Instance\_50\_7.pb} & 3.977 & 13.933 & 0.000 & 0.130 & 81.492 & 0.468 \\
    {Instance\_50\_9.pb} & 3.419 & 10.470 & 0.027 & 0.134 & 85.577 & 0.374 \\
    {Instance\_50\_10.pb} & 3.886 & 9.981 & 0.080 & 0.027 & 85.653 & 0.373 \\
    {Instance\_75\_7.pb} & 6.539 & 19.416 & 0.000 & 0.025 & 73.471 & 0.549 \\
    {Instance\_75\_9.pb} & 7.027 & 16.876 & 0.104 & 0.026 & 75.601 & 0.366 \\
    {Instance\_75\_10.pb} & 7.287 & 15.057 & 0.025 & 0.051 & 77.274 & 0.306 \\
    {Instance\_100\_7.pb} & 8.774 & 26.683 & 0.000 & 0.048 & 63.846 & 0.649 \\
    {Instance\_100\_9.pb} & 9.818 & 22.662 & 0.025 & 0.025 & 66.806 & 0.664 \\
    {Instance\_100\_10.pb} & 9.413 & 22.773 & 0.025 & 0.051 & 67.308 & 0.430 \\
    {Instance\_100\_12.pb} & 9.687 & 21.912 & 0.077 & 0.077 & 67.914 & 0.333 \\
    {Instance\_125\_7.pb} & 11.454 & 34.529 & 0.000 & 0.071 & 53.256 & 0.689 \\
    {Instance\_125\_10.pb} & 12.686 & 28.320 & 0.000 & 0.050 & 58.523 & 0.421 \\
    {Instance\_125\_12.pb} & 12.235 & 23.548 & 0.000 & 0.000 & 63.867 & 0.349 \\
    {Instance\_150\_7.pb} & 12.964 & 38.030 & 0.000 & 0.000 & 48.239 & 0.767 \\
    {Instance\_150\_10.pb} & 14.373 & 33.057 & 0.000 & 0.000 & 52.205 & 0.365 \\
    {Instance\_150\_12.pb} & 15.155 & 31.338 & 0.000 & 0.000 & 53.106 & 0.401 \\
    {Instance\_175\_7.pb} & 15.445 & 43.826 & 0.023 & 0.023 & 40.163 & 0.520 \\
    {Instance\_175\_10.pb} & 16.695 & 38.808 & 0.000 & 0.025 & 43.955 & 0.517 \\
    {Instance\_175\_12.pb} & 18.465 & 37.268 & 0.000 & 0.048 & 43.881 & 0.338 \\
    {Instance\_200\_7.pb} & 17.897 & 47.090 & 0.000 & 0.023 & 34.300 & 0.690 \\
    {Instance\_200\_10.pb} & 19.218 & 42.605 & 0.000 & 0.071 & 37.635 & 0.471 \\
    {Instance\_200\_12.pb} & 18.464 & 41.461 & 0.000 & 0.000 & 39.558 & 0.517 \\
\hline
     \end{longtable}
     \end{center}
     \end{landscape}

